The Impact of Hyperparameters on Large Language Model Inference Performance: An Evaluation of vLLM and HuggingFace Pipelines

The recent surge of open-source large language models (LLMs) enables developers to create AI-based solutions while maintaining control over aspects such as privacy and compliance, thereby providing governance and ownership of the model deployment process. To utilize these LLMs, inference engines are needed. These engines load the model's weights onto available resources, such as GPUs, and process queries to generate responses. The speed of inference, or performance, of the LLM, is critical for real-time applications, as it computes millions or billions of floating point operations per inference. Recently, advanced inference engines such as vLLM have emerged, incorporating novel mechanisms such as efficient memory management to achieve state-of-the-art performance. In this paper, we analyze the performance, particularly the throughput (tokens generated per unit of time), of 20 LLMs using two inference libraries: vLLM and HuggingFace's pipelines. We investigate how various hyperparameters, which developers must configure, influence inference performance. Our results reveal that throughput landscapes are irregular, with distinct peaks, highlighting the importance of hyperparameter optimization to achieve maximum performance. We also show that applying hyperparameter optimization when upgrading or downgrading the GPU model used for inference can improve throughput from HuggingFace pipelines by an average of 9.16% and 13.7%, respectively.

==> datacollectors.tex <==
\subsubsection{Collecting measures from an Inference trial using Data Collectors}
\label{sec:methodology:datacolectors}

In order to compute the dependent variables, we use the following data collectors.
They are executed on each Inference trial.

\paragraph{Nvidia-SMI}
\label{sec:methodology:datacollectors:nvidiasmi}
We use Nvidia-SMI\footnote{} to monitor the activity of the GPUs.
In particular, we collect samples of :
\begin{inparaenum}[\it a)]
    \item Power consumed by the GPU,
    \item  Utilization GPU  (Percent of time over the past sample period during which one or more kernels was executing on the GPU)\footnote{https://enterprise-support.nvidia.com/s/article/Useful-nvidia-smi-Queries-2}.
    \item Utilization memory (Percent of time over the past sample period during which global (device) memory was being read or written)
    \item Total installed GPU memory,
    \item Total free memory,
    \item Total memory allocated.
\end{inparaenum}
These samples are also associated with a \emph{timestamp}, which records the moment the samples are taken.

In case an Inference trial is configured to use more than GPU, we collect the mentioned measures for each of them and then join them together.


\paragraph{MPStats}

MpStats\footnote{\url{https://man7.org/linux/man-pages/man1/mpstat.1.html}} is a Linux tool that provides processors (CPU) statistics.
In particular, we use it to capture the CPUs utilization, which is expressed in a percentage (\%).


\paragraph{CodeCarbon}

CodeCarbon~\cite{courty2024codecarbon} is a framework that reports the energy consumption of a piece of software.\footnote{\url{https://github.com/mlco2/codecarbon}}
Internally, it uses several data collectors, including Nvidia-SMI or RAPL.
We use it to calculate the energy consumed by the processors (CPUs).\footnote{We do not use Nvidia-SMI via CodeCarbon because it does not allow to retrieve the samples of the different measures listed in Section \ref{sec:methodology:datacolectors}.}

==> figInference.tex <==
\begin{figure}[ht]
\centering
\resizebox {0.5\textwidth} {0.5\height} {
\begin{tikzpicture}[node distance=2cm, auto]

% Styles
\tikzstyle{process} = [rectangle, rounded corners, minimum width=3cm, minimum height=1cm, text centered, draw=black, fill=blue!20]
\tikzstyle{arrow} = [thick,->,>=stealth]
\tikzstyle{arrow-dashed} = [thick,dashed,->,>=stealth]

% Nodes for online inference
\node (input1) [process] {Input Request 1};
\node (input2) [process, below of =  input1] {Input Request 2};
\node (input3) [process, below of =  input2] {Input Request 3};

\node (llm1) [process, right of = input2, xshift=2cm] {LLM Inference};

\node (output1) [process, right of = llm1, xshift=2cm] {Output Response 1};
\node (output2) [process, below of =  output1] {Output Response 2};
\node (output3) [process, below of =  output2] {Output Response 3};

% Nodes for batching inference
\node (batching) [process, below of =  input3, yshift=-1cm, text width=4cm] {Batch Input Requests};
\node (llm2) [process, right of = batching, xshift=3cm] {LLM Inference};
\node (batchoutput) [process, right of = llm2, xshift=3cm, text width=4cm] {Batch Output Responses};

% Arrows for online inference
\draw [arrow] (input1) -- (llm1);
\draw [arrow] (input2) -- (llm1);
\draw [arrow] (input3) -- (llm1);
\draw [arrow] (llm1) -- (output1);
\draw [arrow] (llm1) -- (output2);
\draw [arrow] (llm1) -- (output3);

% Arrows for batching inference
\draw [arrow] (input1) |- (batching);
\draw [arrow] (input2) -- (batching);
\draw [arrow] (input3) |- (batching);
\draw [arrow] (batching) -- (llm2);
\draw [arrow] (llm2) -- (batchoutput);

% Dummy nodes for clarity in batch output
\node (dummy1) [right of = batchoutput, xshift=-1cm, yshift=0.5cm] {};
\node (dummy2) [below of =  dummy1, yshift=-0.5cm] {};
\node (dummy3) [below of =  dummy2, yshift=-0.5cm] {};

\draw [arrow-dashed] (batchoutput) -- (dummy1) node[midway,above] {Output Response 1};
\draw [arrow-dashed] (batchoutput) -- (dummy2) node[midway,above] {Output Response 2};
\draw [arrow-dashed] (batchoutput) -- (dummy3) node[midway,above] {Output Response 3};

% Labels
\node[below of=input3, yshift=1.5cm, xshift=-1.5cm] (label1) {Online Inference};
\node[below of=batching, yshift=1cm, xshift=1.5cm] (label2) {Batching Inference};

\end{tikzpicture}
}
\caption{Differences between Online and Batching Inference of a Large Language Model (LLM)}
\label{fig:inferenceOnlineBatch}
\end{figure}

==> ideasTextAndOthers.tex <==
%\textcolor{blue}{RQ1: Which model & config minimize the energy consumption and maximize performance}
\begin{comment}
    "To what degree does the model's structure and parameter count influence energy usage and performance during inference?"
"How does the architecture and scale of the model affect its energy consumption and inference speed?"
"What is the correlation between model architecture, parameter size, and their impact on energy efficiency and inference performance?"
"In what way do the design choices and parameter volume of the model impact its energy efficiency and inference latency?"
"How do variations in model architecture and parameter quantity impact energy consumption and computational speed during inference?"
\end{comment}



%%%%%%%%


Beyond the few lines of code that developers have to write tanks to the abstraction that these libraries provide, there are other challenges for them.
One of them is to establish values for the hyperparameters that these methods have.
From Listing \ref{lstvll1} we observe one in the method that loads the model (\texttt{tensor\_parallel\_size=4}), and two in the inference (\texttt{temperature=0.6} and  \texttt{top\_p=0.95}).
There are two types of hyperparameters: 
\begin{inparaenum}[\it 1)]
    \item those affecting the output of the model inference, such as \texttt{temperature} and  \texttt{top\_p},
    \item other hyperparameters such as \texttt{tensor\_parallel\_size} affecting non-functional properties of the inference such as the speed of inference, represented by metrics as \throughput{} (tokens produced per seconds).
\end{inparaenum}

\todo{something here}
Let us focus on \texttt{tensor\_parallel\_size} which, according to \vLLM{}, is the number of GPUs to use for distributed execution with tensor parallelism.\footnote{\url{https://github.com/vllm-project/vllm/blob/main/vllm/entrypoints/llm.py\#L44C9-L44C29}}
This value has to be put by the developer according to the resources available in the deployment infrastructure.
In \autoref{lstvll1} the value is hard-coded to four. In fact, the initialization of the inference engine \vLLM{} is followed by the following comment:
\emph{\#tensor\_parallel\_size based on the GPUs you are using}.
Listing \ref{lstvllm2} shows a similar real (but simplified) snipped, where the number of GPUs to use is obtained from the environmental variable \texttt{CUDA\_VISIBLE\_DEVICES}\footnote{\url{https://docs.nvidia.com/cuda/cuda-c-programming-guide/index.html\#cuda-environment-variables}}.



%\footnote{\url{https://github.com/MARIO-Math-Reasoning/Super_MARIO/blob/cdc05d1b33745623f3efd714264f195bfe95025b/mcts_math/agents/react.py#L70}}
%Problematic:
\begin{lstlisting}[language=Python, caption=\mbox{},
 basicstyle=\tiny, %or \small or \footnotesize etc.
label=lstvllm2
]
     GPUS = os.environ.get('CUDA_VISIBLE_DEVICES', "0").split(',')
    llm = LLM(model=self.config.model_dir, 
            tensor_parallel_size=len(GPUS), 
            trust_remote_code=True,
            seed=self.config.seed,
        )
\end{lstlisting}


%%%%%%% Inference framewors

According to \hf{} site\footnote{\url{https://huggingface.co/docs/transformers/en/main_classes/pipelines}}: 


\emph{``The pipelines are a great and easy way to use models for inference. These pipelines are objects that abstract most of the complex code from the library, offering a simple API dedicated to several tasks, including Named Entity Recognition, Sentiment Analysis, Feature Extraction.''}

In particular, we are interested in one task: \emph{Text Generation}, which uses the \texttt{TextGenerationPipeline} included in the \hf{} Transformers library\footnote{\url{https://huggingface.co/docs/transformers/en/main\_classes/pipelines\#transformers.TextGenerationPipeline}}.
According to \hf{} \emph{``This pipeline predicts the words that will follow a specified text prompt''}.
Consequently, this task covers our focus: code completion.
\todo{We can use \hf{} without the need of pipeline}
\todo{What about acelerate? \url{https://huggingface.co/docs/accelerate/en/concept_guides/big_model_inference}}  

%% https://huggingface.co/docs/transformers/en/main_classes/pipelines#pipeline-batching
%However, this is not automatically a win for performance. It can be either a 10x speedup or 5x slowdown depending on hardware, data and the actual model being used.





The author measure the 
They test on two types of computation nodes (\nvidia{} A100 and V100).
They evaluated on two datasets: one is the Alpaca dataset \cite{} consists of 52,000 instruction-following tasks, instructions/questions where some have example inputs and some do not, that the model is asked to answer. 
The second dataset is GSM8K \cite{} consisting of 8,500 human crafted grade school math problems.

In the first RQ, the authors study the performance of the models, expressed in Words/Second metric.
In that experiment, for each model, inference is made with a batch size of 64 and a maximum generation length of 256. 
The found remarkable differences between the hardware uses (A100 is more efficient), except for the 65B model.
Then, they also compute the energy per second (in watts).
They observe that the improvement of the thoughput by using A100 seen previoysly is not for free: the energy per second also increase.

They continue by analyzing just one model: Llama 65B.
They used four batch sizes: 64, 128, 256 and 512, with a max gen equals to 512 and 1024 tokens.
Overall, They see an average increase in energy per second with the number of shards. While there is a slight correlation as energy per second increases with increasing batch size, increasing the number of shards always increases the wattage.
Here, they use just the  we mainly use V100 GPUs for larger- scale distributed experiments (i.e., for 8, 16, and 32 shards)

After they focus o the energy per decoded token.
 the number of shards increases, the energy per output token also increases.
 As with energy per second, max generation length seems to have a negligible effect on energy costs from 512 to 1024.
there exists a “sweet spot” at 16 shards where continuously increasing the batch size can actually reduce the energy per token at max generation length 512. 
However, this disappears under max generation length 1024 where increasing the batch size increases the energy per token
Then, they focus on the energy per response.

we see that increasing the number of shards still tends to increase the energy costs of inference per response most overall while increasing the maximum generation length from 512 (Figure 8) to 1024 (Figure 9) does not induce a clear or significant effect in inference energy costs.

while we see slight increases in energy costs per response generated within a shard configuration as batch size increases, but not consistently or significantly.

They also do power capping experiment and GPU Resource Utilization under Distributed Inference.



%%%%%%%



%\subsection{Other hyperparameters to optimize}
other hypermarameter temp
Some of them has an impact on the output.
For example, seed,  
Temperature also has an impact,
Precision: 


%In fact, 
%There are two types of hyperparameters: 
%\begin{inparaenum}[\it 1)]
    \item those affecting the output of the model inference, such as \texttt{temperature} and  \texttt{top\_p},
    \item other hyperparameters such as \texttt{tensor\_parallel\_size} affecting non-functional properties of the inference such as the speed of inference, represented by metrics as \throughput{} (tokens produced per seconds).
\end{inparaenum}


Latency: There is a trade-off between batch size and latency. While larger batch sizes can improve throughput, they may also introduce higher latency for individual requests, especially in real-time systems


%more engines from from https://www.anyscale.com/blog/continuous-batching-llm-inference
FlashAttention.
%https://huggingface.co/docs/transformers/perf_infer_gpu_one



%%% \documentclass[10pt,conference]{IEEEtran}
%\documentclass[sigconf,review]{acmart} 
\usepackage{graphicx} 
\usepackage{comment}
\usepackage{enumerate}
\usepackage{xcolor}
\usepackage{subcaption}
\usepackage{paralist}
\usepackage{mdframed}
%%Added
\usepackage{url}
\usepackage[hidelinks]{hyperref} 
\usepackage{booktabs} 
\usepackage{amsmath}
\usepackage{listings}

\newmdenv[
  backgroundcolor=gray!20,
  linewidth=0pt,
  innertopmargin=3pt,
  innerbottommargin=3pt,
  innerleftmargin=5pt,
  innerrightmargin=5pt,
]{graybox}

\pagenumbering{arabic}
\pagestyle{plain}

\usepackage{tikz}
\usetikzlibrary{shapes.geometric, arrows}

\usepackage{tabularx}
\usepackage{xspace}
\newcommand{\todo}[1]{\textcolor{red}{#1}}
\newcommand{\hpo}{hyperparameter optimization\xspace}
\newcommand{\approachhpo}{\texttt{InfPop}\xspace}
\newcommand{\llm}{LLM\xspace}
\newcommand{\hf}{HuggingFace\xspace}
\newcommand{\nvidia}{Nvidia\xspace}
%\newcommand{\hfinference}{\texttt{HuggingFace pipeline+A\xspace}}
\newcommand{\hfinference}{\texttt{HF$_{pl}$\xspace}}
\newcommand{\vLLM}{\texttt{vLLM\xspace}}
\newcommand{\hfsig}{HF\xspace}

\newcommand{\throughput}{throughput\xspace}


\newcommand{\ts}{t/s\xspace}



\title{
%Hyperparameter Optimization of HuggingFace and vLLM inference Libraries for Code Completion\todo{\throughput{}}
%Performance of vLLM and huggingFace inference 
%Performance Evaluation and Optimization of Large Language Model Inference: A Case Study of \vLLM{} and HuggingFace Pipelines for Code-Completion Tasks
%%% Candidates 
%The Impact of Hyperparameters on LLM Inference Performance: A Comparative Evaluation of \vLLM{} and HuggingFace pipelines for code-completion task"
The Impact of Hyperparameters on Large Language Model Inference Performance: An Evaluation of vLLM and HuggingFace Pipelines% for Code-Completion Tasks
%%% and optimi
%The Impact of Hyperparameters on Large Language Model Inference Performance: An Evaluation and optimization of \vLLM{} and HuggingFace Pipelines for Code-Completion Tasks
%"Optimizing Throughput in Large Language Models: A Comparative Study of \vLLM{} and HuggingFace's Pipelines
%The Impact of Hyperparameters on Large Language Model Inference Performance: An Evaluation of \vLLM{} and HuggingFace Pipelines for Code-Completion Tasks

%%The Role of Hyperparameters in Large Language Model Performance: Evaluation and Optimization with \vLLM{} and HuggingFace Pipelines for Code-Completion
%Performance Evaluation and Optimization of Large Language Model Inference: The Role of Hyperparameters in \vLLM{} and HuggingFace Pipelines for Code-Completion Tasks"
}
\author{Anonymous}
%\date{November 2023}

\begin{document}

\maketitle

%\newcommand{\rqshapespace}{What is the shape of the throughput response within the hyperparameter space defined by number of GPS and batch size? Does this shape exhibit constant values, peaks, valleys, or flat regions?}

\newcommand{\rqshapespace}{RQ1: What is the shape of the throughput landscape across the hyperparameter space defined by the batch size and the number of GPUs on \vLLM{} inference?}

\newcommand{\rqonlineinferenceHFGPU}{RQ2: For online inference, how does throughput vary with different numbers of GPUs (hardware scaling)?}


\newcommand{\rqBatchInference}{RQ3: For batched inference, how does throughput vary with the batch size?}



\newcommand{\rqOlderHardare}{%RQ4: What is the impact of using older -previous-generation- GPU hardware?
%RQ4: What is the impact of the GPU hardware ?
RQ4: How does \throughput{} vary between different GPU models during inference?
%RQ4: How does the \throughput{} of the inference tasks vary across different GPU models?
%How does \throughput{} of the inference vary according to the GPU model used?
}


\newcommand{\rqHPO}{RQ5: To what extent does applying Hyperparameter Optimization improve \throughput{} in \llm{}?}

\begin{abstract}
   % The current wave of open source large language models (LLM) allow developers to create AI-based solutions while controlling different aspects such as privacy, and compliance, providing them governance and ownership of the deployment process. 
    
   % To interact with these LLMs, inference engines are required, which are in change of loading the model (i.e., its weights) on the available resources and to then execute the inference (i.e., given the query, execute the model to produce an output).

   % The speed of inference or performance of the LLM inference critical for real-time applications,as it has to compute millions or billions of floating point operations per each inference. 

  %  Recently, inference engines, such  which implement novel inference mechanism, as \vLLM{}  have emerged to provide state-of-the-art performance.

   % In this paper, we study the performance (in particular, the \throughput{}) of 20 LLMs using two popular inference libraries: \vLLM{} and \emph{pipelines} from HuggingFace.
   % In particular,  we focus on how hyperparameters, that developers have to set, affect on the  performance of inference.

  %  Our results show that the \throughput{} landscapes are irregular (e.g., have peaks), involving that hyperparameter optimization is capital to achieve maximum performance.
  %  We also present a study showing that applying hyperparameter optimization in a scenario of upgrading or downgrading the GPU model used for inference helps to increase \throughput{}, on average up to 13.7\%. 

The recent surge of open-source large language models (LLMs) enables developers to create AI-based solutions while maintaining control over aspects such as privacy and compliance, thereby providing governance and ownership of the model deployment process.
To utilize these LLMs, inference engines are needed. These engines load the model’s weights onto available resources, such as GPUs, and process queries to generate responses.
The speed of inference, or performance, of the LLM, is critical for real-time applications, as it computes millions or billions of floating point operations per inference.
Recently, advanced inference engines such as \vLLM{} have emerged, incorporating novel mechanisms such as efficient memory management to achieve state-of-the-art performance.
In this paper, we analyze the performance, particularly the \throughput{} (tokens generated per unit of time), of 20 LLMs using two inference libraries: \vLLM{} and HuggingFace's \emph{pipelines}. We investigate how various hyperparameters, which developers must configure, influence inference performance.
Our results reveal that \throughput{} landscapes are irregular, with distinct peaks, highlighting the importance of hyperparameter optimization to achieve maximum performance.
We also show that applying hyperparameter optimization when upgrading or downgrading the GPU model used for inference can improve \throughput{} from HuggingFace pipelines by an average of 9.16\%  and  13.7\%, respectively.
    
\end{abstract}

\begin{comment}
https://conf.researchr.org/track/icse-2025/icse-2025-research-track
    
    i) Novelty: The novelty and innovativeness of contributed solutions, problem formulations, methodologies, theories, and/or evaluations, i.e., the extent to which the paper is sufficiently original with respect to the state-of-the-art.

ii) Rigor: The soundness, clarity, and depth of a technical or theoretical contribution, and the level of thoroughness and completeness of an evaluation.

iii) Relevance: The significance and/or potential impact of the research on the field of software engineering.

iv) Verifiability and Transparency: The extent to which the paper includes sufficient information to understand how an innovation works; to understand how data was obtained, analyzed, and interpreted; and how the paper supports independent verification or replication of the paper’s claimed contributions. Any artifacts attached to or linked from the paper will be checked by one reviewer.
\end{comment}


\section{Introduction}
\todo{cite in the intro \cite{bai2024beyond}\cite{li2024llm}}

%Yarally2023BatchingGreenAI
%The batch size (i.e., the number of input data
%samples that are processed at one time during inference) is
%one of the most important hyperparameters to tune during the
%training phase. It has implications on the model accuracy and
%generalisability [5], training times and parallelisability [13],
%etc.


Xhou et al. \cite{zhou2024survey} survey on efficient inference  for LLMs, which  targets different aspects, from providing primary causes of
the inefficient LLM inference to  defining comprehensive taxonomies of, for instance, inference engines.
In particular, they analyze features from inference engines including the two we consider, \hfinference and \vLLM{}
They also conducted experiments such as the evaluation of the speed-ups achieved
by employing uantization techniques on two models LLaMA-2-7B and 13B using two inference frameworks, TensorRT-LLM\cite{}  and LMDeploy\cite{}. 
Recent advances on inference are also discussed in \cite{li2024llm}
%They used a single single NVIDIA A100 GPU and 
\cite{miao2023towards} survey

\cite{shi2024efficient} to cite, importan vision paper.

\cite{white2023navigating} 
`` The directions highlighted in this section are just examples of the opportunities afforded by the emergence of generative AI and copilots in search settings. There are other areas for search providers to
consider too, such as multilingual copilot experiences (i.e., foundation models are powerful and could help with language translation
[33, 74]), copilot efficiency (i.e., large model inference is expensive and not sustainable at massive scale, so creative solutions are
needed [72]), the carbon impact from running foundation models
at scale to serve billions of answers for copilots [18], making copilots private by design [70],``


\todo{\cite{yang2024robustness} no mention any hpo work on LLM}


\todo{\cite{miao2023towards} survey inference, different to the other}

%\todo{check survey LLM for codegen\cite{jiang2024survey}}


%We are living a era where  artificial intelligence is changing many professions, including software engineering.
%The maner of developers build, test, deploy and maintant has also radicaly change since the apareance of these large language models.

%We are living a era where  artificial intelligence allows developers to do tasks quite 
\todo{High throughput serving of large language models (LLMs)
requires batching sufficiently many requests at a time (vllm paper)}

\todo{\cite{ghadesi2024causes} hyperparameter in SO including HF post.}

Large language models (LLM) have revolutionized the manner in which developers build \emph{intelligent} software solutions, impacting several areas, including most of the software engineering (\cite{}).
One of the main actors from this revolution are the \emph{open-source} LLMs. 
which has publicly accessible architecture, code, checkpoint (model weights) and, eventually, training data.
Open-source LLMs enables developers to create AI-based solutions while maintaining control over aspects such as privacy and compliance, and, at the same type, providing governance and ownership of the model deployment process.
%
The current success of open-source in AI, including open-LLM, could be attributed to platforms such as \hf{} (\hfsig), which offers more than 700.000 models available for download, including state-of-the-art models such as CodeLlama~\cite{roziere2023codellama}.
%

Inference engines (or frameworks) are software components that make LLMs operable.
They have as main responsibility to load the model's weighs into the available devices (GPU and/or CPU), and to make the \emph{inference} i.e., to generate a prediction, output, response based on input data.
\hf{}, for instance, provides inference mechanisms into its \texttt{Transformer} library~\cite{wolf-etal-2020-transformers}, for example \texttt{pipelines}, which are objects that abstract complex code used for inference (wraps other libraries such as Pytorch) and offer a simple API dedicated to several tasks, including text generation.

%The appearance of open-source \llm{} encourages this latter strategy, as a developer can download a model, modify it (e.g. applying fine-tuning, pruning, quantization, or other techniques) and then deploy it in a desired infrastructure as those mentioned.
%For example, \hf{} (\hfsig), the platform that drives open-source initiatives on AI,  has more than 700.000 models available for download.
%To applying this strategy, the developers need an inference engine, which is a piece of software that has as main responsibility to load the model into the available devices (GPU and/or CPU), and then to query it (i.e., to perform the inferences).
%Among all the functionalities and features provided by \hf, there are two that simplify the integration of \llm{} into apps, available on library \texttt{Transformer}~\cite{wolf-etal-2020-transformers}.
%The first one, \texttt{AutoModel.from\_pretrained(<model\_id>)}, downloads and loads a model on the available devices.
%Then, \hf{} provides different methods for performing inference on that loaded model, such as \texttt{pipelines}, which offer a simple API dedicated to several tasks, including text generation.
%For instance, \hf{} provides \texttt{pipelines}, which are objects that abstract complex code used for inference (which wraps other libraries such as PyTorch) and offer a simple API dedicated to several tasks, including Text-Generation.
%\hf{} pipelines simplifies the manner to integrate and use \llm{} within software application.  

A key factor for the success of an inference engine is \emph{performance}, because it directly impacts the user experience of AI-powered systems.
%Inference engines are critical components in the deployment of \llm{} into real-world applications. 
%Their performance directly impacts the user experience of AI-powered systems.
A measure of LLM performance is \emph{\throughput{}}, expressed in tokens generated by \llm{} per unit of time.
%Measurement of the performance of an inference engine involves evaluating various metrics such as \emph{\throughput{}}, expressed in tokens generated by an \llm{} per unit of time.
%This metric represents the number of inferences that the inference engine can process per unit of time or, in the case of text generation tasks, the amount of text (expressed as the number of tokens) per unit of time that \llm{} can generate.
%High throughput indicates the engine can handle a large volume of requests efficiently or can generate t.
With the goal of improving the performance of the inference process, inference engines have recently emerged~\cite{miao2023towards,zhou2024survey}, for example, \vLLM{}~\cite{kwon2023efficient}, a memory-efficient inference engine for \llm{}, launched in June 2023.
Inference engines such as vLLM or HuggingFace can be integrated into applications with a few lines of code, as \autoref{lsthf1} shows.
However, the inference engine has hyperparameters that developers need to set by the developers.
Listing \ref{lsthf1} shows a real utilization of \hf{} pipelines\footnote{\url{https://github.com/adit-copilot/EnchantedQuest/blob/48d6256c482abc40a8c916c6c8d1a7c5edb2c6fa/retrival/qa_pipeline.py\#L46}}, which first loads the model (it has one hyperparameter \texttt{device\_map}) and then creates a pipeline with the model as a parameter. % together with other hyperparameters (e.g,  \texttt{max\_new\_tokens}). 
Listing~\ref{lstvll1} shows  real code (but simplified)  that uses \vLLM{}\footnote{\url{https://github.com/tencent-ailab/persona-hub/blob/5e9b7d0a29eff2e2eaf01cc8c74d4abb731fb4a0/code/vllm\_synthesize.py\#L37}}. 
The first line loads the model (with hyperparameter \texttt{tensor\_parallel\_size}), the second performs inferences from a list of prompts (receives two hyperparameter \texttt{temperature} and  \texttt{top\_p}).


\begin{lstlisting}[language=Python, caption=\mbox{\hf{}},
 basicstyle=\tiny, %or \small or \footnotesize etc.
label=lsthf1
]
    model = AutoModelForCausalLM.from_pretrained(model_name, device_map='auto',[...])
    return pipeline("text-generation", 
        model=model, 
        max_new_tokens=100,
        model_kwargs={"torch_dtype": torch.bfloat16} [...]
    )
\end{lstlisting}





\begin{lstlisting}[language=Python, caption=\mbox{\vLLM{}},
 basicstyle= \tiny, %or \small or \footnotesize etc.
label=lstvll1
]
    llm = LLM(model=model_path, tensor_parallel_size=4)
    #tensor_parallel_size based on the GPUs you are using
    outputs = llm.generate(prompts, SamplingParams(temperature=0.6, top_p=0.95, [...]))
\end{lstlisting}


%From the listings we observe that both libraries have \emph{hypermarameters}.
%Listing \ref{lstvll1} shows three, one used on model load  (\texttt{tensor\_parallel\_size=4}) and other two are used during inference (\texttt{temperature=0.6} and  \texttt{top\_p=0.95}).


There are hyperparameters that have a direct incidence in \throughput{} while others do not (for example, \texttt{temperature} affects the output of an \llm{}).
%
{{In this paper, we study the impact of hyperparameters on \throughput{}.}}

Before continuing, let us briefly describe some of these hyperparameters.
\texttt{tensor\_parallel\_size} from \vLLM{} is the number of GPUs to use for distributed execution with tensor parallelism.\footnote{\url{https://github.com/vllm-project/vllm/blob/main/vllm/entrypoints/llm.py\#L44C9-L44C29}}
The \texttt{tensor\_parallel\_size} value needs to be set by the developer according to the resources available in the deployment infrastructure.
In \autoref{lstvll1}, \texttt{tensor\_parallel\_size} is hard-coded to 4. In fact, the initialization of the inference engine \vLLM{} is followed by the following comment:
\emph{\#tensor\_parallel\_size based on the GPUs you are using}.
Both \texttt{from\_pretrained} and \texttt{pipeline} form \hf{} have a similar hyperparameter, named \texttt{device\_map},  which indicates the devices (GPU, CPU) to use.
In Listing\ref{lsthf1}, \texttt{device\_map} receives the value \texttt{auto}, which means that \hf{}  automatically determines the deployment of the model depending on the available resources. %CUDA_VISIBLE_DEVICES


Another of these hyperparameters that affect \throughput{} is \emph{batch size}, which refers to the number of input instances processed simultaneously by the model in a single inference call. 
Increasing the batch size typically increases throughput.
However, this is subject to the limitations of the memory capacity of the hardware (e.g., GPU is not able to allocate the memory of numerous inputs).
On the other hand, a low value may lead to hardware being underutilized.
For example, \autoref{lsthf2batch} shows a snippet from a real app\footnote{\url{https://github.com/mlcommons/inference/blob/c3c68ee61896e1e4d74b096565b627e14422337d/language/mixtral-8x7b/SUT.py\#L130}}
 that sets the \texttt{batch\_size} with the value given by the user, but if it is not provided, the default value $32$ is set. 

\begin{lstlisting}[language=Python, caption=\mbox{},
 basicstyle=\tiny, %or \small or \footnotesize etc.
label=lsthf2batch
]
     if not batch_size:
            if device == "cpu":
                batch_size = 1
            else:
                batch_size = 32  # Reduce to 8 if using 4 GPUs, 16 for 8.
        self.batch_size = batch_size
\end{lstlisting}

%\todo{Choosing an appropriate batch size $n$ is challenging.
%On the one hand, a high value of batch size would lead optimize the resource (GPU) utilization and, consequently, increase the throughput, expressed in tokens per second.
%However, at the same time, a high batch size may lead to an out-of-memory exception: for example, the GPU is not able to allocate the memory of numerous inputs.
%On the other hand, a low value may lead to resources (e.g., GPUs) being underutilized.}


The problem is that \llm{} have different hardware (GPUs) and memory requirements (e.g., VRAM memory). For instance, some LLMs need to be distributed across multiple GPUs to manage their size and the computational load.
Consequently, letting developers choose and set hyperparameter values, especially the number of GPUs and batch size, may have negative effects on the inference performance. 


The final goal of our research is to equip developers with approaches and tools for hyperparameter optimization to achieve high-performance inference.

In this paper, we first study how hyperparameters of inference engines affect  the \throughput{}of \llm{}.
In particular, we examine the throughput landscape defined by the spaces of two hyperparameters, the number of GPUs and batch size.
We study it in the context of code generation: we exercise \llm{} with the code completion task, where each inference consists of completing the code given as input. 

In our experiment, we consider 20 open-source \llm{}, all from key players in the AI industry such as Meta, Google, Microsoft, Mistral and HuggingFace, 
and we use \hfinference{} and \vLLM{} as inference engines.
The experimental infrastructure used is equipped with 8 GPUs \nvidia{} A100 and 8 \nvidia{} V100, which are devices used to train and evaluate most of the \llm{} under consideration.


The results shows 

\todo{}



We also present an approach for hyperparameters optimization.


The paper continues as follows.
Section \ref{}.
Section \ref{}.
Section \ref{}.
Section \ref{}.
Section \ref{}.
Section \ref{}.







%https://github.com/mlcommons/inference/blob/c3c68ee61896e1e4d74b096565b627e14422337d/language/mixtral-8x7b/SUT.py#L8

% https://github.com/neulab/prompt2model/blob/d4cd23d50c8f5edc5755ab487bcee18121d42a4f/prompt2model_demo.py#L426

%Inference libraries have hyperparameters.
%Not sure how to configure to maximize a property such as \throughput{}

%https://github.com/search?q=%22from+vllm+import+LLM%22+language%3APython+&type=code&p=5







%\url{https://github.com/adit-copilot/EnchantedQuest/blob/48d6256c482abc40a8c916c6c8d1a7c5edb2c6fa/retrival/qa_pipeline.py#L46}
%\url{https://github.com/liminma/pdfChat-Llama2/blob/bd6810bf35871bc0fad7ba4ebc383206a163331a/app/src/pdf_chatbot.py#L28}
%\url{https://github.com/pgalko/BambooAI}
%\url{https://github.com/digitalfabrik/integreat-qa-dataset/blob/57cbbbd7d8e5751164f96587dbed340ec4f9e825/tools/get_answers_llm.py#L114}



% text-generation-inference (we dont use it)
%https://huggingface.co/docs/text-generation-inference/quicktour
%https://huggingface.co/docs/text-generation-inference/supported_models




%https://huggingface.co/docs/transformers/en/main_classes/pipelines#pipeline-batching
%However, this is not automatically a win for performance. It can be either a 10x speedup or 5x slowdown depending on hardware, data and the actual model being used.


%%% https://huggingface.co/docs/transformers/v4.15.0/en/performance

%\medskip
%\begin{graybox}
%The challenge of this paper is to hyperoptimize parameters (in particular the number of GPUs and batch size) in order to improve the throughput  two inference libraries: \hfinference{} and \vLLM{} 
%\end{graybox}






%% https://github.com/tencent-ailab/persona-hub/blob/5e9b7d0a29eff2e2eaf01cc8c74d4abb731fb4a0/code/vllm_synthesize.py#L37

%%https://github.com/MARIO-Math-Reasoning/Super_MARIO/blob/cdc05d1b33745623f3efd714264f195bfe95025b/mcts_math/agents/react.py#L70












%\subsection{memory}


%\todo{As batch size increases, the model processes more tokens in parallel, leading to higher throughput. This is typical behavior for many models where larger batch sizes improve parallel processing efficiency.
%This is likely due to the saturation of GPU resources such as memory bandwidth and compute units.
%At larger batch sizes, the overhead and inefficiencies associated with managing very large batches might start to outweigh the benefits, leading to diminishing returns in throughput gains.}


%Choosing an appropriate batch size $n$ is challenging.
%Choosing a high value, a developer attempts to optimize the resource (GPU) utilization and, consequently, increase the throughput expressed in tokens per second.
%It has two main drawback:
%\begin{inparaenum}[\it 1)]
%    \item setting a high batch size may conduct to an out-of-memory exception: for example, the GPU is not able to allocate the memory of numerous inputs.
%    \item In the domain of our study (code auto-complete), it could affect the latency: given $z$ requests to autocomplete a batch size of $n>1$,  the \llm processes the \todo{}.
%    To avoid that, vLLM implements a novel \todo{continue}. 
%\end{inparaenum}
%In contrast, choosing a low value may lead to a resource under utilization.





\section{Research questions}
\label{section:rq}

The research questions that guide this experiment are the following:
%\medskip
\begin{graybox}
\rqshapespace
\end{graybox}


The goal is to visually inspect, for each of the \llm{} under study, the throughput distribution within the hyperparameter space defined by the number of GPUs and batch size with the goal of analyzing its shape.
In particular, we search for:
\begin{inparaenum}[\it 1)]
\item[] peaks, 
\item[] flat regions, or
\item[] valleys.
\end{inparaenum}

This analysis gives us the first sing to know whether hyperparameter optimization should be applied to maximize or minimize a property, such as  \throughput{}.
For example, a peak in the landscape is a sign that there is a set of hyperparameters that maximize the throughput.

%Once we perform the visual analysis, in the subsequent research questions we apply a series of numerical analysis in order to quantify the impact of hyperparameter changes on the \throughput{} under certain conditions, including type of inference, inference engine, and hardware used.


%\medskip
\begin{graybox}
\rqonlineinferenceHFGPU
\end{graybox}


The purpose of this question is to study the impact of the number of GPUs on \throughput{}.
This question could help us to know, for example, whether having more GPUs in the inference infrastructure (called \emph{GPU scaling}) allows an inference engine to improve \throughput{}.
%The number of GPUs is one hyperparameter of some inference engine, including the two, \vLLM{} and \hfinference{}, presented in Section \ref{sec:backgroud}.
%Here, we study the relation between that hyperparameter space and the \throughput{}.

In this research question, we focus on \emph{online inference}, 
each query done to the model (i.e., a request) through the inference library includes just one input. As a result, the model generates one output (or eventually more than one if applying, for example, beam search) for that single input.

%The alternative to \emph{online inference}  is \emph{batching}, which  consists in sending multiple inputs in a single query. 
%The inference produces, as a response to that query, one or more outputs of each of the inputs included in the query.
%We study the impact of batching in RQ3.

%Figure \ref{fig:inferenceOnlineBatch} shows the differences between online and batching inference processes.
%\input{figInference}.
%\todo{explain}.



%\medskip
\begin{graybox}
\rqBatchInference
\end{graybox}

This research question focuses on the \emph{batch} inference. 
In contrast to the previous one, where the query to the \llm{} consists of one \emph{single} input, the batching considers $n$ inputs in a single query.
This $n$ is the \emph{batch size}, which is an hyperparameter of the inference processes. 
Choosing an appropriate batch size $n$ is challenging.
On the one hand, a high batch size value would lead to throughput improvements but also may lead to an out-of-memory exception.
On the other hand, a low value may lead to resources (e.g., GPUs) being underutilized.
Here, we study the relation between the space of the hyperparameter batch size and the \throughput{} from inference engines.

%Choosing an appropriate batch size $n$ is challenging.
%On the one hand, a high value of batch size would lead optimize the resource (GPU) utilization and, consequently, increase the throughput, expressed in tokens per second.
%However, at the same time, a high batch size may lead to an out-of-memory exception: for example, the GPU is not able to allocate the memory of numerous inputs.
%On the other hand, a low value may lead to resources (e.g., GPUs) being underutilized.


%\medskip
\begin{graybox}
\rqOlderHardare
\end{graybox}
%\medskip


Each new generation of GPUs boasts improved performance including \throughput{} \cite{Choquette2021NvidiaA100}.
In this research question, we measure the variation in  \throughput{} across two GPU models, one representing a recent and widely used model, and another model from a previous generation. 


%\medskip
\begin{graybox}
\rqHPO
\end{graybox}
%\medskip


The goal is to present an use case in which \hpo{} of \llm{} inference produces improvements in \throughput{}.
In particular, we apply \hpo{} (using our approach \approachhpo{}) in cases where there are changes on the hardware infrastructure used for inference.
Thus, \hpo{} finds a new  hyperparameter values that maximize \throughput{} on the new hardware.




\section{Experimental protocol}
\label{sec:methodology:experimentalprotocol}


In order to answer the research questions, we conduct an experiment that consists of executing the code-completion task for a set of incomplete programs. 
That completion is done by doing inference calls to a \llm{} using an inference engine. 
%The inference of the missing code is done via an inference engine, which loads the model on the available devices (e.g., CPU, GPUS) and executes the queries on it.

This section introduces all steps to carry on our experiment, and continues as follows.
Section \ref{}
Section \ref{} presents the criteria to select the \llm{} to evaluate.
Section 
\todo{to complete}
We detail them in Section \ref{sec:methodology:dataset}




\subsection{Selection of the inference engines to evaluate}
\label{sec:methodology:selectionInferenceengine}

%% https://github.com/search?q=%22from+vllm+import+LLM%22+language%3APython+&type=code

We evaluate the \throughput{} from the code-completion task conducted using two inference engines: \hf{} inference and \vLLM{}.

\subsubsection{Inference  from \hf{} Transformers library}
We select it for the following reasons.
First, it offers  simple, easy to use, and concise APIs to perform inference on \llm{}.
For example, \emph{pipelines} abstracts most of the complex code from the library, and provides a simple API dedicated to several tasks, including Text Generation. An example for this pipeline  is shown in \autoref{lsthf1}.
% shows a pipeline for the ``text generation'' tasks, which englobe our specific task (code completion).
Internally, that code uses a pipeline \texttt{TextGenerationPipeline}. 
%, included in the HF Transformers library\footnote{\url{https://huggingface.co/docs/transformers/en/main\_classes/pipelines\#transformers.TextGenerationPipeline}}. 
In the remainder of the paper, we will refer to the HuggingFace pipeline for text generation it as \hfinference{}.
Secondly, \hf{} provides thousads of models which can be used with  \hfinference{} for inference.
Lastly, HF Transformers has is a relevant library in the  the scene of open-source on AI: it has $\approx$130.000 stars on GitHub.
%We choose to study the inference method provided \hf{} for the relevance that it has in the scene of open-source on AI: HF Transformers has $\approx$130.000 stars on GitHub.


\subsubsection{\vLLM{}}
 originaly materialized to implement  \emph{PagedAttention}~\cite{kwon2023efficient} a technique  for efficient management of attention key and value memory of transformer architecture. 
%Other key features from \vLLM{} include:
%\begin{inparaenum}[\it 1)]
 %   \item Continuous batching of incoming requests,
 %   \item A wide range of Quantization techniques (GPTQ, AWQ, SqueezeLLM, FP8 KV Cache), and
 %   \item optimized CUDA kernels.
%\end{inparaenum}
We choose to study \vLLM{} for different reasons, including:
\begin{inparaenum}[\it a)]
   \item It provides state-of-the-art inference performance on \llm{}~\cite{kwon2023efficient}.
	\item introduces a novel memory management (PagedAttention)~\cite{kwon2023efficient}, then integrated to other inference engines \cite{li2024llm} such as TensorRT-LLM \todo{cite}.
    \item It integrates with \hf{} models, enabling it to work with state-of-the-art LLMs.
    \item Popularity: more than 23.000 Github stars since its launch (June 2023).
    \item Well integrated with other \llm{} libraries and frameworks such as LangChain\footnote{\url{https://python.langchain.com/v0.2/docs/integrations/llms/vllm/}},  SkyRocket\footnote{\url{https://docs.vllm.ai/en/latest/serving/run_on_sky.html}} which facilitates its adoption.
\end{inparaenum}






\subsection{Selection criteria of the \llm{} to evaluate}
\label{sec:methodology:selectionLLMs}

\input{tables/tabLLMInfo}
%During recent years, researchers and companies have released numerous deep learning models capable of understanding and generating source code~(e.g., \cite{jiang2024survey,yang2024ecosystemLLMonCode,zhang2023survey,zhang2023unifying}).
%In this work, we focus on autoregressive models, particularly those based on the Transformer architecture~\cite{vaswani2017attention}. 
%This architecture is highly effective for code auto-completion tasks due to their ability to generate sequences token-by-token, maintaining context and dependencies \cite{Svyatkovskiy2020IntelliCode}.

The model selection criteria are the following:
\begin{itemize}
    \item The model is based on the Transformer architecture~\cite{vaswani2017attention}, which is effective for code completion tasks~\cite{Svyatkovskiy2020IntelliCode}. %due to their ability to generate sequences token-by-token, maintaining context and dependencies \cite{Svyatkovskiy2020IntelliCode}.
    \item As our study focuses on large language models (LLM), the model must have $\approx >$1 billion parameters.%\footnote{Determining when a model is ``large" is quite arbitrary, as there is no strict size threshold on the number of parameters, architectures or amount of data used in training.}
    %\item fully or partially trained with source code.
    \item Evaluated on HumanEval~\cite{chen2021evaluating} to demonstrate their competence in the code generation task.
    \item Open-source models: model weights (checkpoints) are available on the HuggingFace hub\footnote{HuggingFace model hub: \url{https://huggingface.co/models}}.
    \item The model architecture is implemented in the \texttt{HuggingFace Transformers} library\footnote{Model architectures implemented in HuggingFace transformer library: \url{https://github.com/huggingface/transformers/tree/14ff5dd962c1bd0a4e3adaac347ba396d8df5add/src/transformers/models} and \url{https://huggingface.co/docs/transformers/}}~\cite{wolf-etal-2020-transformers} or this library is able to load models that it does not include.\footnote{Possible using option \texttt{trust\_remote\_code=True} in method \texttt{from\_pretrained} from class \texttt{AutoModelForCausalLM}.}
    \item In the \hf{} site of the model, it  is tagged with ``Text-Generation"\footnote{\url{https://huggingface.co/models?pipeline_tag=text-generation}}  tag. This ensures that it can be used with the HF pipeline.   
    \item The model is supported by the vLLM library.
\end{itemize}

To select the models to study, we first inspect the vLLM documentation and its Github repository to detect the supported models.
As \vLLM{} uses HuggingFace Transformers library, this strategy allows us to select models supported by both the \hfinference{}  and \vLLM.
For each supported model, we read its documentation, related paper, HuggingFace model card, and the dashboard Paper-on-Code\footnote{\url{https://paperswithcode.com/sota/code-generation-on-humaneval}} in order to 
verify if it meets all the mentioned criteria.


Table \ref{tab:model_data} shows the 20~\llm{} that meet the criteria mentioned above and work in our infrastructure.
It shows the numbers of parameters, which range from 1.3 to 70 billions, and the HumanEval (pass@1) reported by the models's authors. 
We include \llm{} from key players in the AI industry, such as Meta (\cite{roziere2023codellama}), Google (\cite{team2024gemma}), Microsoft (\cite{gunasekar2023textbooksPhi_1,Li2023Phi1_5},) Mistral~ (\cite{jiang2023mistral,jiang2024mixtral}), and HuggingFace\footnote{HuggingFace participates via BigCode:  \url{https://www.bigcode-project.org/}} (\cite{li2023starcoder,lozhkov2024starcoder}).
Other models are discarded because do not fulfill some of the criteria. For example, 
Moisaic~\cite{MosaicML2023Introducing}, Command-R and Aya from Cohere4AI have not been evaluated on HumanEval;
CodeGen \cite{nijkamp2022codegen}, Incoder~\cite{fried2022incoder} are not supported by vLLM at the time of preparing this article (July 2024),
Another model,  Microsoft Phi-3, was discarded because we failed to deploy it due to an instalation problem with its dependency FlashAttention\footnote{https://github.com/Dao-AILab/flash-attention}.


\subsection{Evaluation benchmark}
\label{sec:methodology:dataset}

HumanEval \cite{chen2021evaluating} is a dataset of 164 handwritten programming problems proposed by OpenAI to evaluate functional correctness and measure the problem-solving capabilities of their code-based models.
%In particular, \cite{chen2021evaluating} evaluated the ability of their model Codex to generate correct Python functions given as input a \texttt{docstring} i.e., a description of the program to generate.
%Programming tasks in the HumanEval dataset assess language comprehension, reasoning, algorithms, and simple mathematics.
%We consider HumanEval as it has been one of the most used benchmarks for code generation (e.g. code \llm{} from Meta, Google and Microsoft use it).
We consider HumanEval as it has been used by  big AI players (e.g., OpenAI, Meta, Google, Microsoft) to evaluate the capaibilities of their LLMs.

Researchers created new benchmarks  from HumanEval, to evaluate other tasks beyond function generation.
For example, Fried et al.~\cite{fried2022incoder} and Bavarian et al.~\cite{bavarian2022efficient} evaluated code \emph{infiling} task, which consists of predicting missing text spans that are consistent with the preceding and subsequent code.

To evaluate the code completion task, we select  \emph{Single-line infilling}\footnote{\url{https://github.com/openai/human-eval-infilling/blob/88062ff9859c875d04db115b698ed4b0f0395170/data/HumanEval-SingleLineInfilling.jsonl.gz}}~\cite{fried2022incoder}.
They created it by marking out each non-blank line of code in the canonical function implementation from each HumanEval problem. %, creating N examples for a function with N non-blank lines per problem.
In total, \emph{Single-line infilling} contains 1033 examples. 
%Each of these examples has:
%\begin{inparaenum}[\it a)]
  %  \item a masked line,
   % \item the code that precedes the masked line,
    %\item the code that is subsequent to the masked line.
%\end{inparaenum}
We use this bechmark in a slightly different manner:
we query a model to generate code just based on the preceding code, and we ignore the subsequent code as code completion is not infilling.
%We do not asset the correctness of the generated code because it is not within the scope of this paper.



\subsection{Hardware used}
\label{sec:methodology:hardware}

We use two high-performance computation nodes available in our host infrastructure:  two CPU Intel Xeon E5-2698 and 512 GB of RAM.
The first one is equipped with eight \nvidia{} A100 GPUs with 40 GB ~\cite{Choquette2021NvidiaA100} .
We choose this node because that GPU has been extensively used to train and evaluate state-of-the-art LLMs considered in our study. 
The second node is equipped with a GPU model from a previous generation: \nvidia{} V100\footnote{\nvidia{} V100 whitepaper: \url{https://images.nvidia.com/content/volta-architecture/pdf/volta-architecture-whitepaper.pdf}}, which is the first Tensor Core GPU introduced by \nvidia{} designed specifically for deep learning.
The node is equipped with eight  V100 with 32 GB.
We choose to include V100 in our experiment as a ``previus generation'' GPU because it has been also used to train and evaluate some LLMs considered in this study (e.g.  Bloom~\cite{workshop2022bloom}).

%Tesla V100-SXM2-32GB 
%https://www.nvidia.com/en-us/data-center/v100/

%Tesla V100-SXM2-32GB 
%https://www.nvidia.com/es-es/data-center/tesla-v100/




\subsection{Executing Inference trials on the Single-line infilling}
\label{sec:methodology:vars}
\label{sec:methodology:inference}
%\input{tables/tabVariables}

We call a \emph{trial} to the execution of the code completion tasks for all items from the  \emph{Single-line infilling} benchmark by querying one \llm{}  $m$, using an inference engine $e$ ($e \in [\hfinference{},\vLLM])$, executed on $n$ GPUs  ($n \in [1, 2, 4, 8]$)  of model $g$ ($g \in [A100, V100]$), with a batch size $b$ ($b \in [1, 2, 4, 8, 16, 32, 64, 128, 256, 1028]$). 
We run \emph{trials} resulting from all the combinations between $m$, $e$, $n$, $g$ and $b$.
Note that, for each \emph{trial}  with batch size $b$, we create $x$ inference invocations, each with $b$ elements from the benchmark ($x$ results from the division between the size of the benchmark and $b$). 
%For example, if the batch size is 4, we create 258 batches (1033 / 4) and the inference is then invoked for each of them.
In \vLLM{}, we  modify the parameter of  the  constructor of class \texttt{LLM}. 
\texttt{tensor\_parallel\_size} for pasing the number of GPUs to be used, and pass $b$ queries to the method  \texttt{generate} from that class, where $b$ is the batch size of the trial.
In \hfinference{},  we keep \texttt{device\_map="auto"} from the pipeline and, at the same time, we restringe the visible GPUs by changing the  evironmental variable \texttt{CUDA\_VISIBLE\_DEVICES}.
For example, for a trial that uses 2 GPUs, we set the value \texttt{0,1}. Then, the other GPUs ($2\dots8$) are not visible.
This strategy allows the pipeline, thanks to the \texttt{auto} configuration provides by the HF Accelerate library, to determine automatically the model deployment  on the available (and visible) devices.
For the batch size, we pass the value $b$ via hyperparameter \texttt{batch\_size} from the pipeline.


%https://huggingface.co/docs/accelerate/v0.32.0/en/concept_guides/big_model_inference
%(https://huggingface.co/transformers/main_classes/pipelines.html#pipeline-batching

We keep the default values for the other hyperparameters from the inference engine,  except for two.
First, we indicate the inference engine to generate up to 5 tokens.
Second, we unify the floating-point precision used.
All models from \autoref{tab:model_data} use by default half-precision floating point (FP16/float16) with the exception of one (bigcode/starcoder2-3b) which uses full-precision floating point (FP32/float32).
To ensure a fair comparison between models and engines, we explicitly set the hyperparameter precision to FP16 in both inference engines as is the value from the large majority.
\todo{versions of vllm and transformer?}
For each trial, we calculate \throughput{} as the number of tokens generated during the trial (composed by $x$ inference invocations) divided by the execution time of the trial in seconds (\ts{}).


\subsection{Data analysis to answer the research questions}
\label{sec:methodology:rq}

Once executed all trials, we apply the following analysis to answer each research question.

%\subsubsection{\rqshapespace}
\subsubsection{RQ1}
We plot the \throughput{} landscapes using the Python library matplotlib. There is a plot for each combination of:
\begin{inparaenum}[\it a)]
    \item hardware,
    \item inference engine, and 
    \item \llm{}.
\end{inparaenum}
We then inspect the shape of all the landscapes to select the representative cases for discussion.


%\subsubsection{\rqonlineinferenceHFGPU}
\subsubsection{RQ2}


We select the trials with batch size equal to one.
Then, for each \llm{}, we plot the \throughput{} evolution with different numbers of GPUs, and report the number of GPUs that maximize \throughput{}. 
We test the hypothesis \emph{$H_0$:~there is no statistically significant difference in throughput across different numbers of GPUs} by appling an analysis of variance (ANOVA).
In this test, each group  corresponds to the trial with the same number of GPUs used on inference (1, 2, 4 and 8).
Finally, we compare \throughput{} between the two inference engines, \vLLM{} and \hfinference{}.


%\subsubsection{\rqBatchInference}
\subsubsection{RQ3}


For each combination of 
\begin{inparaenum}[\it a)]
\item inference engine, \item  GPU model, \item  number of GPUs, and  \item \llm{}, 
\end{inparaenum}
we plot the evolution \throughput{} with the batch size. 
Then, for each of them, we test the null hypothesis  \emph{$H_0$: There is no a significant difference in the throughput values based on the batch size} using  ANOVA.

%\subsubsection{\rqOlderHardare}
\subsubsection{RQ4}

To compare the \throughput{} obtained with a \nvidia{} A100 with that one obtained with a \nvidia{} V100, we  first compare the \throughput{} from pairs of trials, one from A100, the other from V100, but sharing the other hyperparameters (\llm{}, batch size, number of GPUs).
%This comparison is done using Eq.\ref{eq:improvementhard}:
%\begin{equation}
%\label{eq:improvementhard}
%\text{I$_{it}$} = \left( \frac{\text{throughput$_{it}$ A100} - \text{throughput$_{it}$  V100}}%{\text{throughput$_{it}$ on V100}} \right) \times 100
%\end{equation}
Moreover, we compute, for each inference engine, the Wilcoxon Signed-Rank Test to test the null hypothesis \emph{$H_0$:~The difference in \throughput{} between Nvidia A100 and v100 is not significant}.


%\subsubsection{\rqHPO}
\subsubsection{RQ5}
\label{sec:protocol:hpo}

We evaluate the impact of \hpo{} in two experiments: 
\begin{inparaenum}[\it 1)]
\item Upgrading and
    \item Downgrading  GPU. 
\end{inparaenum}
Both consider two GPUs models, \emph{previous} (P) and \emph{new} (N).
For studying the \emph{Upgrading}, P becomes the \nvidia{} V100 model, and N is \nvidia{} A100.
For \emph{Downgrading}, P is A100 and N is V100.
%Then, both experiment shares the same steps, with the difference on the values of N and P.
Each experiment is as follows.
For each pair \llm{} and inference engine, we  search the set of hyperparameters $HP_{orig}$ that maximize \throughput{} on P.
Then, we measure \throughput{} of using $HP_{orig}$ on N.
After that, we apply \hpo{} on N to find new hyperparameters $HP_{best}$ that maximize \throughput{} on N.
Finally, we compare \throughput{} from $HP_{best}$ and $HP_{orig}$  to measure the impact of \hfinference{}.


%subsubsection{Hyperopt \cite{Bergstra2015Hyperop}} is a distributed asynchronous hyper-parameter optimization framework, based on the Tree-of-Parzen-Estimators (TPE) algorithm \cite{Bergstra2011AlgorithmsHyper}.
%TPE is a Bayesian optimization approach~\cite{Shahriari2015}, based on \emph{Sequential Model-Based Optimization}~\cite{Hutter2011smbo}), which builds a probability model $p(score|hyperparameter)$ (aka the ``surrogate'' function) of the objective fitness function and uses it to select the most promising hyperparameters to evaluate in the objective function. 

To apply \hpo on inference engines, we implement \approachhpo{} (\underline{Inf}erence hyper\underline{P}arameter \underline{Op}timization).
Internally,  \approachhpo{}  uses Hyperopt~\cite{pmlr-v28-bergstra13Hyperopt}, a state-of-the-art \hpo{}, used  hyperoptimizing other software engineering tasks~\cite{lustosa2023optimizingSNEAK,martinez2023DAT}.
\approachhpo{} receives as input: 
\begin{inparaenum}[\it 1)]
\item a list of queries to pass to a LLM (in our experiment, queries for code-completion from the \emph{Single-line infilling} benchmark),
\item a specification of the hyperparameter space. In this experiment, we consider two hyperparameters: number of GPUs and batch size.
\item a \emph{objective/fitness function}: In this study, \approachhpo{}'s function aims at maximizing the \throughput{} of performing inference on the mentioned queries.
\end{inparaenum}
\approachhpo{} produces as output a set of values for the hyperparameters that allows the inference engine to maximize the objective (\throughput{} in this experiment).
%
%\todo{For a matter of space, we provide more details in our appendix.}


We hyperoptimize \vLLM{} and \hfinference{} on each \llm{}. 
Given the stochastic nature of Hyperopt, we conduct each experiment 10 times and report the average results.




\section{Results}
\label{sec:results}

%%%%%%% RQ 1

\subsection{\rqshapespace}


\input{figshapes}

Figure \ref{fig:landscapes} shows six plots, each corresponding to an LLM and an inference engine. In Appendix~\cite{appendix} we include all of them, including interactive versions that facilitate the visualization and analysis.
Two axes represent the hyperparameter space: batch size and number of GPUs, while the third one -the vertical one- corresponds to the throughput.
%These plots represent \todo{common} shapes that we observed between all plots generated.
This analysis does not aim to perform a rigorous classification of these shapes, but to provide evidence though these examples, that the throughput landscapes are not uniform, thus hyperparameter optimization would be useful. 

Figure \ref{fig:plot:space:a100_autohf_Bloom-1b7} shows the Bloom-1b7 landscape using \hfinference{}.
It has two peaks where the throughput is much higher ($\approx94.5$) than in other parts of the landscape (between 60 and 70 t/s): one uses one GPU and another uses eight GPUs, both with batch size 64.
Increasing that increasing the batch size above 64 produces memory errors.
%Reducing the batch size (from 64 up to 2) or using 2 or 4 GPUs significantly reduce the throughput (between 60 and 70 t/s).


The second case, Fig. \ref{fig:plot:space:a100_autohf_Codellama-7b-hf}, shows the landscape for CodeLlama and \hfinference{}. 
It presents different peaks, most notably:
\begin{inparaenum}[\it 1)]
\item  one single GPU and and batch size 16,
\item two GPUs and batch size 64, and
\item four GPUs and batch size 128.
\end{inparaenum}
This shows that for CodeLlama when one increases the GPUs, the batch size should be also adjusted.
This case also shows the challenging of determining optimal hyperparameter values:
Codellama-7B using one single GPU can infer batches up to size 16. Putting values of 32 or greater produces memory errors.

The third case, Fig. \ref{fig:plot:space:a100_autohf_Mistral-7b} corresponds to Mistral-7b  and \hfinference{}.
It has a peak at one GPU and batch size 32. Greater batches with one GPU cause memory errors. 
Beyond this peak, the landscape presents a descending inclined plane as the batch enlarges. 
The landscape also exhibits high values of throughput (similar to the mentioned peak) with four GPU and small batches (4 and 8).
With 4 GPUs, increasing the batch size decreases the throughput.


The fourth case, 
Fig. \ref{fig:plot:space:vLLM_Gemma-2b} corresponds to Gemma-2 and \vLLM{}.
We observe that:
\begin{inparaenum}[\it 1)]
  \item There is a significant improvement of throughput when using 4 or 8 GPUS compared to using 1 or 2 GPUs.
 \item The landscape has a \emph{plateau}: a vast zone where the values are relatively constant, do not change significantly throughout the plateau, and represent a high-throughput region. We can observe it in yellow.
This plateau is located in the region bounded by 4 to 8 GPUs and batch sizes ranging from 128 to 1024.
  \item The throughput given with eight GPUs is slightly higher than that with four.
 \item The highest throughput is with a batch size equal to 258: increasing the size slightly impacts throughput. However, the reduction is more evident when the batch size is smaller than 258.
 \end{inparaenum}



%The fifth case, Fig.\ref{fig:plot:space:autohf_Codestral-22b} corresponds to CodeStral-22b and \hfinference{}.
%It produced results with 4 and 8 GPUs, but not for \todo{1 or 2}.
%The plot shows a flat region that maximizes throughput for batch sizes between 4 and 16.
%Neverteless, given a particular batch size, the throughput given with four GPUs is slightly higher than those with eight. 

The fifth case, Fig. \ref{fig:plot:space:a100_autohf_Starcoder} corresponds to Starcoder-15b and \hfinference{}.
It has a peak with one GPU and batch size 32 and increasing the batch size to a value just greater than the peak produces a memory error.
However, this landscape has two main differences with respect to the two previous examples.
First, it has a second peak when using two GPUs and a larger batch size (128).
Secondly,
the throughput landscape shows a downward slope, indicating that throughput decreases as the number of GPUs increases.

{\bf\emph{Hardware specifics.}}
The previous landscapes resulted from the execution of inference on a computing node equipped with \nvidia A100. %, one of the most widely used hardware to train the evaluated model.
We also inspect the landscape resulted from the  V100.
Even in the majority of cases the landscapes from both models produces similar shapes (A100 shapes have higher peaks, i.e. higher throughput, because it is a more recent and advanced model), others exhibit more noticeable differences.
For example, Fig.~\ref{fig:plot:space:tesla_autohf_Starcoder} shows the execution of StarCoder-15b in a V100 (the Fig at its left shows the landscape of this model from A100).
We observe that the shape is different: there is not a peak but a thin and long plateau region bounded by 2 and 8 GPUs batch sizes 8 and 16.
This means that, a \llm{} is deployed in a another GPU model,
it might be necessary to adjust the hyperparameters in order to maximize the throughput.
In RQ5 we study this.


%\medskip
\begin{graybox}
%Visual inspection of the throughput landscape from  inference using \hfinference{} and \vLLM{} shaped by different hyperparameter values shows that the throughput is sensitive to hyperparameter and GPU hardware. 
Visual inspection of the throughput landscape from  inference using \hfinference{} and \vLLM{} shows irregular landscapes, some with marked peaks.
Consequently, to assure a maximization of the \throughput{} for a particular inference engine and hardware infrastructure would require an inspection of the landscape.
\end{graybox}
%\medskip



%In the rest of this paper,  we perform a detailed, quantitative study, focusing on specific \throughput{} values to derive precise insights and statistical significance.

%Scaling Efficiency
%Communication overhead: With multiple GPUs, inter-GPU communication can become a bottleneck, especially as you scale up.


%Memory constraints: Larger batch sizes require more GPU memory, which can be a limiting factor.
%Scaling efficiency: As you increase the number of GPUs, you'll want to monitor how well the throughput scales (linear scaling is ideal but rarely achieved in practice).
%Communication overhead: With multiple GPUs, inter-GPU communication can become a bottleneck, especially as you scale up.
%Hardware specifics: Different GPU models and interconnect technologies can significantly impact performance.



%%%%%%%%%%%%%%%% ONLINE:

\input{tables/tabHFvLLMOnline}
\input{figOnlineHFGPUs}


\subsection{\rqonlineinferenceHFGPU}



\autoref{tab:minMaxMetricAutoHFVLLMOnlineInferece}  and \autoref{fig:onlineGPUsAutoHFvLLM} show the throughput of online inference performed by \hfinference{} and \vLLM{} when scaling \nvidia{} A100 GPUs.
The table shows: 
\begin{inparaenum}
    \item for \hfinference{}, the number of GPUs that maximizes the \throughput{} for each model (column Best),
    \item for \vLLM{}, in column Same, the \throughput{} using that number of GPUs (for a fair comparison),
    \item for \vLLM,  the number of GPUs that maximizes the \throughput{} for each model (column Best).
\end{inparaenum}
Tables showing the \throughput{} per GPU, and the results from V100 can be found in our appendix~\cite{appendix}.

%Let us start the analysis by analyzing the figures. 
We observe that the scaling hardware when using \hf{} has a different effect than when using \vLLM{}. All findings also apply for Nvidia V100.
%For this reason, we study them separately.

\subsubsection{\bf \vLLM{}}
From \autoref{fig:gpus_evol_a100_vLLM_throughput}  we identify two primary observations.
\begin{inparaenum}
    \item[] First, scaling  from 1 to 2 GPUs using \vLLM{} has a strong (negative) impact on \throughput{} of some models (e.g., Microsoft Phi-1), even for others (such as CodeLlama-13b) has a moderate (positive) impact.
    \item[] Second, scaling from 2 to 4, and then from 4 to 8 GPUs has less impact on \throughput{}: the plot shows that the \throughput{} of most of the model is bounded between 60 and 80 \ts{}. 
\end{inparaenum}

We also observe:
\begin{inparaenum}[\it a)]
    \item with one GPU, \throughput{} presents a large variability in the models: it goes from 32.5 to 171.5 \ts{}.
    This variability is reduced after scaling.
    \item 8 models with $\le$ 3 billion parameters  maximize \throughput{} using a single GPU,  
    \item when scaling to two GPUs, there are two effects: the first one is that \throughput{} dramatically drops (which is the case for the ``smaller'' models previously mentioned); the second one is the \throughput{} slinging vary positively in most of  models with 13-15 billion parameters.
    \item  Models with 7-13 billion parameters maximize \throughput{} using 4 GPUs. %Thus, \todo{scaling up to 4 GPS has a negative impact for these models}
    \item  Models with more than 15 billions parameters typicaly maximize \throughput{} with 8 GPUS.
    %\item The largest models we evaluated (e.g., CodeLlama-34b, WizardCoder-33b) maximize \ts{} with 8 GPUs (in total, 6 models, see column \texttt{\vLLM{}-Best}). 
    %However, reducing the scale does not cause substantial losses \ts{} 
    %(e.g., the \throughput{} from StarCoder-15b  is 57 and 58.4 for 4 and 8 GPUs respectively).
   % In this case, the developer and/or manager and/or infrastructure leader need to assess the value of scaling up – and the additional cost of resources – to achieve those extra throughput points and consider how this could lead to increased business value.

\end{inparaenum}


\paragraph{\bf Statistical test for \vLLM{}}
%We performed a hypothesis test to determine whether the throughput values differ significantly according to the number of GPU uses.
%We perform an analysis of variance (ANOVA) as we have multiple groups, each for a number of GPUs used on inference (1, 2, 4 and 8).
Taking into account all GPUs, the ANOVA test rejects the null hypothesis $H_0$ at the significant level $\alpha =  0.05$ (F-statistic: 5.44, p-value: 0.002) which indicates that there is a statistically significant difference in throughput across different numbers of GPUs for both A100 and V100 GPUs.
We suspect that this significant difference is dragged by one of the analyzed groups, GPU 1, which maximizes \throughput{} for some \llm.
For that, we performed two additional tests. First, the re-execution of the ANOVA test by just considering trials with 2, 4 and 8 GPUs  failed to reject $H_0$.
Secondly,  Tukey HSD test (Honestly Significant Difference) reveals significant differences in performance metrics between using GPU 1 and each of the other groups (2, 4, and 8). However, no significant differences were found between GPUs 2, 4, and 8. 
%which provides a pairwise comparison of the means of different groups to determine if their differences are statistically significant.
%The test results reveal significant differences in performance metrics between GPU 1 and GPUs 2, 4, and 8. However, no significant differences were found among GPUs 2, 4, and 8. 




\subsubsection{\bf \hfinference{}}
From  \autoref{fig:gpus_evol_a100_autohf_throughput}, we observe two major differences with respect to \vLLM{}:
\begin{inparaenum}[\it 1)]
    \item the \throughput{} are lower than using \vLLM{}, independently of the number of GPUs used;
    \item when scaling, there is no dominant pattern evolution of \throughput{} as for \vLLM{}.
\end{inparaenum}
Moreover:
\begin{inparaenum}[\it a)]
\item Scaling GPU results in a very slight decrease of \throughput{} from  models with ~7b parameters  (Bloom-7B1, CodeLlama-7b, Mistral-7b).
\item The decline is more pronounced in StarCoder2-3b. 
\item Scaling cause down and up (e.g., Bloom-1b7, Bloom3-b).
\item Scaling cause up and down (e.g., Phi-1, Phi-2).
\end{inparaenum}
In conclusion, using the  \hfinference{}, scaling generally does not improve throughput for most LLMs (with few exceptions such as  Phi-1 and Gemma-7). 

\paragraph{\bf Statistical test for \hfinference{}}


Based on the results of the ANOVA test, we cannot reject the null hypothesis ($H_0$) at the 0.05 significance level (F-statistic: 0.37, p-value: 0.77). This means that there is not enough statistical evidence to suggest that the means of the groups -number of GPUs- are significantly different, which can be translated as scaling up GPUs does not produce significant changes in \throughput{}.


\subsubsection{\bf Comparison between Inference Engines}
Table \ref{tab:minMaxMetricAutoHFVLLMOnlineInferece} shows the \throughput{} for each model (columns \texttt{Thp}) and the improvement in \throughput{}.
Taking into account the number of GPUs that led \hfinference{} to maximize \throughput{} (column \texttt{\vLLM{} Same}), \vLLM{} achieves a mean (median) improvement of 4.3$X$  (6.47$X$).
%
However, for 12 LLMs, \vLLM{} maximizes \throughput{} by using a different number of GPUs (column \texttt{\vLLM{} Best}), 
achieving a mean (median) improvement of 7.26$X$ (4.80$X$) with respect to \hfinference{}.
In nine of these 12 cases, \vLLM{} achieves the gain by using more GPUs and, in the remaining three cases, fewer GPUs.
This shows that both \vLLM{} and \hfinference{} need to be optimized separately, at least on the number of GPUs, to increase \throughput{}.

The reason behind the difference in \throughput is that \vLLM{} was designed to achieve fast inference, that is, state-of-the-art serving throughput.
For that, \vLLM{} introduces key improvements. We briefly discuss two of them.
First, \vLLM{}  uses \emph{PagedAttention}~\cite{kwon2023efficient},  a new attention algorithm that manages the attention keys and values from the Transformer architecture \cite{vaswani2017attention}.
In autoregressive decoding, all the input tokens to the LLM produce their attention key and value tensors, and these tensors are kept in GPU memory to generate the next tokens. 
This has several problems for LLMs, such as the large amount of memory required and memory waste~\cite{kwon2023vllmBlog}. 
PagedAttention proposes a solution inspired by the idea of virtual memory and paging in operating systems: it allows storing continuous keys and values in noncontiguous memory space.
The second improvement is \emph{Continuous batching}, initially proposed by~\cite{Orca2022Batching}.
During inference, instead of waiting until every sequence in a batch has completed generation (as traditional static batching does) this approach, once \emph{a sequence} in a batch has completed generation, a new sequence is inserted in its place. This yields a higher resource utilization than static batching \cite{vllmcontinousbatching} and thus increases \throughput{}.


% https://huggingface.co/docs/transformers/perf_infer_gpu_one
%https://huggingface.co/blog/bloom-inference-optimization


%\medskip
\begin{graybox}
{\bf \underline{Answer to RQ2:}} 
For \vLLM{}, GPU scalability benefits larger LLMs ($\approx$13 billion parameters or more), maximizing \throughput{} with the use of eight GPUs. However, scaling up GPUs penalizes smaller models ($\approx$ 3 billion parameters or fewer), decreasing their \throughput{}. For these smaller models, the optimal configuration is using 1 or 2 GPUs.
In contrast, using \hfinference{}, scaling hardware does not significantly increase \throughput{} for most of the LLMs studied. 
Additionally, on the same hardware, \vLLM{} achieves an average \throughput{} that is 6.47 times higher than that of \hfinference{}.
\end{graybox}
%\medskip



%\medskip
\begin{graybox}
{\bf \underline{Implications:}}
 \hfinference{}{} may conduct to under-optimal results when the node has more than one GPU (since it uses all GPUs).
Furthermore, we recommend hyperoptimizing the number of GPUs to be used during inference. 
%and explicitly pass this parameter rather than, for instance, using the \texttt{auto} on hyperparameter \texttt{device\_map}.
\end{graybox}
%\medskip



%%%%%%% RQ 3
\subsection{\rqBatchInference}



\input{figBatchesAll}

We study how the \throughput{} varies according to the batch size by using a particular number of GPUs.

\subsubsection{\bf \hfinference{}}

\autoref{fig:batchesA100} shows the \throughput{} using 1, 2, 4 and 8 \nvidia{} A100 GPUs  and \hfinference{.}
We observe:
\begin{inparaenum}[\it a)]
    \item The four plots show similar trend.
     \item Scaling on hardware (more GPUs) allow to have larger batches. 
The reason is that there is more memory on the GPU to allocate bigger batches and thus compute more inputs in parallel.
  \item the maximum \throughput{} is usually reached with the largest batch size that correctly works. For example, Phi-1 achieves the maximum \throughput{} with a batch size 64, larger batches produce memory errors. 
  %   \item for some \llm, increasing the batch size has a impact on the \throughput{}, for example, StarCoder-15.
     
\end{inparaenum}

\paragraph{\bf Statistical test for \hfinference{}}

We compute the ANOVA test for each group of GPU configurations (1, 2, 4, and 8).
For both  \nvidia{} A100 and V100, we reject the null hypothesis $H_0$ for 1, 2 and 4 GPUs, at the significant level $\alpha=0.05$. All p-values are shown in our appendix.
In contrast, we cannot reject $H_0$ when the trial has eight GPUs.
%We hypothesize that the increase of GPUs to eight also entails having more memory to process larger batch sizes and, consequently, .
\todo{here improve}

\input{figBatchSize}

\subsubsection{\bf \vLLM{}}

\autoref{fig:RQ3_bs_throughput_a100_autohf} shows the \throughput{} obtaining with different batch sizes and using two GPUs.
The plots for one, four, and eight GPUs exhibit the similar trend and are available on our appendix \cite{appendix}.
From these plots, we observe that:
\begin{inparaenum}[\it 1)]
    \item Throughput generally increases with batch size across most models.
    \item The improvement is more noticeable for smaller to medium batches (up to 128).
   \item Most models achieve their highest throughput around batch sizes of 64 to 256. 
   Beyond this point, throughput tends to plateau, indicating that increasing batch size further does not significantly improve throughput.
   \item For some models, such as Starcoder-15b and Gemma-2b, after the plateau, the \throughput{} shows a slight, but not significant, decrease.
   \item  Moreover, for Bloom-1b7 (as well as for other models using 4 or 8 GPUS) the \throughput{} shows a slight decrease followed by a subsequent increase.
\end{inparaenum}
All these points mean that optimizing the batch size is crucial to maximize \throughput{} in \llm{}. 
when using \vLLM{} inference.



\paragraph{{Statistical test}}

For both types of hardware, \nvidia{} A100 and V100, and for each number of GPU, we reject the null hypothesis $H_0$ at the significant level $\alpha=0.05$ (p-values listed in appendix).


\subsubsection{Comparison \hfinference{} and \vLLM{}}

\autoref{fig:batchsizes2GPU} shows the \throughput{}  from \hfinference{} and \vLLM{} both using two \nvidia{} A100 GPUs)
We observe that:
\begin{inparaenum}[\it a)]
    \item with batch size 1, in both engines the \throughput{} is below to 100 \ts{}.
    \item However,  \throughput{}  from \vLLM{} increases rapidly with batch size. For \hfinference{} the increase is moderate for some models (e.g., Phi-1, Bloom-1b7) or null for others (CodeLlama-7b).  
    \item Starcoder-2-3b with \hfinference{} outperforms the other models and has a huge increase from batch size 4.
     \item Since batch size 4, the \throughput{}  from \vLLM is between 100 and almost 800 \ts{}. In contrast, for \hfinference{}, with the exception of the Starcoder-2-3b mentioned above, \throughput{} never passes 100 \ts{}.
\end{inparaenum}
These findings also apply for the inference using 1, 4 and 8 GPUS and GPU \nvidia{} V100.


\paragraph{{Statistical test}}

We apply Wilcoxon Signed-Rank Test to test the null hytothesis $H_0$: 
\emph{The difference in throughput between \vLLM{} and \hfinference{} is not significant.}
For all number and model of GPUs, the test rejects $H_0$ at the 0.05 significance level (all p-values are in our appendix).
Moreover, we measure the effect size employing Cliff's delta ($\delta$) in order to quantify the magnitude of differences between the \throughput{} from \vLLM{} and \hfinference{}.
Across all all number and model of GPUs evaluated, the mean $\delta$ is 0.8762.
This indicates a very large effect size, suggesting a significant difference between the two groups,  with \vLLM{}  scoring higher than \hfinference{}.



%\medskip
\begin{graybox}
{\bf \underline{Answer to RQ3:}} 

In \hfinference{}, increasing the batch size leads to slight or moderate increases in \throughput{} for some models (e.g., CodeLlama-7b) and steep increases for others (e.g., Bloom-1b7).
Increasing the size of the batch that maximize the \throughput{}  often results in out-of-memory errors.
Scaling up GPUs allows \hfinference{} to process larger batches.
Conversely, increasing \vLLM{} significantly impacts small to medium batches (fewer than 64). For larger batches, the changes in \throughput{} are not substantial and not conduct to out-of-memory errors. 
%\vLLM{} has significantly higher \throughput{} than \hfinference{} in the two hardware devices tested.
Overall, \vLLM{} achieves significantly higher \throughput{} than \hfinference{} on the two hardware devices tested.
\end{graybox}
%\medskip

%\todo{Bad things of increasing the batch size in bt}

%\medskip
\begin{graybox}
{\bf \underline{Implications:}} 
Optimizing batch size is crucial to maximize \throughput{} in \llm{}. 
In \hfinference{}, determining the optimal batch size and number of GPUs to achieve maximum \throughput{} is challenging because is bonded by the GPU memory. %due to the limitations imposed by \nvidia{} GPU memory.
%ecause it is bounded by the \nvidia{} GPU memory.
This insight is valuable for hyperparameter optimization, especially in scenarios where throughput is a critical performance metric.
\end{graybox}
%\medskip


\subsection{\rqOlderHardare}


%\input{tables/tabHardwareComparison}

%We compute the differences of \throughput{} between \nvidia{} A100 and V100. 
For \vLLM{}, the increase of \throughput{} using A100 compared to V100 is on average 83.5\% (median 77.6). 
The models that exhibit the largest difference are Gemma-7b, Codellama-13b, 34b and 70b, Wizardcoder-15b, all with 100\% or greater improvement by using A100.
%We did not detect a correlation between model size and improvements, e.g. WizardCoder-33b shows a 57.4\% of improvement, improvement similar to a smaller model, Phi-1\_5 with 51.4\%, but lower than a model with similar number of parameters Codellama-34b with 114.1\%.
Appendix \cite{appendix} includes a detailed table with the improvement for each model and hardware. 

We compute Wilcoxon Signed-Rank Test to test the null hypothesis $H_0$: 
\emph{The difference in throughput between \nvidia{} A100 and V100 is not significant} for \vLLM{}. We reject $H_0$ at the significant level $\alpha = 0.05$  (p-value = 2.01).
We measure the effect size to quantify the differences of \throughput{} between A100 and V100 using Cliff's delta~\cite{cliff1993dominance}. A delta value of 0.406 suggests a moderate effect size, indicating a moderate difference between A100 and V100 using \vLLM{}.

For \hfinference{}, the increase of  \throughput{}  using A100 is lower on average, 47\% (median 23.3\%).
Notally, the increase is greater  for the largest models such as WizardCoder-33b (535.6\%) and Codellama-70b-hf (276\%), but smaller for the small models such as Gemma-2b (1.9\%),  Phi-2 (21.8\%).
We reject $H_0$  for \hfinference{} at the significant level $\alpha = 0.05$ (p-value = 3.88).
The measurement of effect size using Cliff's delta is 0.1333, which indicates a small but noticeable effect accross   \throughput{}  from A100 and V100. 



\begin{graybox}
{\bf \underline{Answer to RQ4:}} 
Upgrading (or downgrading) the GPU model (i.e., from a \nvidia{} V100 to A100) has a significant impact on the throughput of \vLLM{}, with an improvement of 83.5\% on average) and on \hfinference{} with an improvement of 47\% on average.

\end{graybox}


\begin{graybox}
{\bf \underline{Implications:}} 
Developers of AI-based systems need to analyze the following trade-off, either:
\begin{inparaenum}[\it a)]
    \item  {\underline {Maximizing Throughput}}: Opt for the \nvidia A100 to achieve maximum throughput. This choice involves higher costs due to the premium price of state-of-the-art hardware; or % driven by high demand from the AI boom.
\item  {\underline {Reducing Operational Costs}}: Choose older hardware like \nvidia{} V100, which might result in lower throughput but eventually reduce operational expenses. This option is particularly advantageous for LLMs where difference of throughput accross A100 and V100 is modest (e.g., \hfinference{} and small LLMs such as Microsoft-Phi and Google-Gemma).
\end{inparaenum}
\end{graybox}




\subsection{\rqHPO}
\label{sec:rqhpo}

\input{figHPO}

Fig \ref{fig:violinhpo} shows the distribution of improvement on the \throughput{} given by the new  hyperparameter values found by our tool \approachhpo{},  in the context of GPU upgrade (from \nvidia{} V100 to A100) and downgrade (from  A100 to V100).
For upgrading, the optimization produces \hfinference{} a median (avg) increase in the \throughput{} of 6.4\% (9.16\%).
For some models, e.g., Starcoder-15 the improvement is higher (24\%), while for others three there is not improvement (i.e., the best configuration, in terms of \throughput{}, of \hfinference{} on V100 is also the best on A100).
For downgrading, improvements are, on the median, 5.61\% (average 13.7\%).
For \vLLM{} the improvements are lower, in both upgrading (median 3.3\%) and downgrading (median 6.9\%).
The reason is that, as shown in \autoref{fig:RQ3_bs_throughput_a100_vLLM}, the evaluated hyperparameters in \vLLM{} have less impact on \throughput{} than in \hfinference{}.



\begin{graybox}
{\bf \underline{Answer to RQ5:}} 
Our results suggest that applying hyperparameter optimization during changes in the inference infrastructure —such as upgrades or downgrades of GPU devices— can yield improvements in throughput. On average, \hpo{} enhances throughput from \hfinference{} by 9.16\% during GPU upgrades and 13.7\% during GPU downgrades.
\end{graybox}

\begin{graybox}
{\bf \underline{Implications:}} 
Applying \hpo{} during hardware upgrades (e.g., GPU) is crucial to maximize the benefits provided by the new hardware. Applying \hpo{} during hardware downgrades is essential because the transition from a newer model (A100) to an older one (V100) typically results in a decrease in \throughput{}. 
This study demonstrates that \hpo{} can help to mitigate these performance losses.
%\todo{re-tuning}


\end{graybox}




\section{Discussion}
\label{sec:discussion}


\subsubsection{{Deployment of LLMs on available hardware}}

%\todo{REASONS for scalling decrease the results}
%\todo{It first  use the maximum space available on the GPU(s)
%if we still need space, we store the remaining weights on the CPU}
%https://huggingface.co/docs/accelerate/v0.32.0/en/concept_guides/big_model_inference


Both \vLLM{} and \hfinference{} inference engines are able to deploy  ``big'' \llm{} using the CPU and just one GPU.
The reason is that these engines provide specially mechanism, such as HF Accelerate \cite{accelerate} activated via the hyperparameter   \texttt{device\_map="auto"}, to  determine automatically where to put each layer of the model depending on the available resources.
In the case of Accelerate, it first uses the maximum space available on the GPU(s), when, 
iit still need space, it store the remaining weights on the CPU, RAM, and finally on the hard drive as memory-mapped tensors.
For example,  Starcoder2-3b and 2-7b, Bloom-1b7, 3b and 7b1, CodeLlama-7b, gemma-2b, phi-1\_5
Mistral-7B-v0.1 fits in one GPU (either A100 or V100) without the need of extra space on the GPU.
From Table \ref{tab:minMaxMetricAutoHFVLLMOnlineInferece} we observe that this configuration maximizes their  \throughput{}.
The other models can do the inference with 1 GPU as weights are stored in GPUs and, for Mixtral, also on the disk, damaging the \throughput{}.
This is a clear example that having more GPUs negatively impacts on \hfinference{} when using  \texttt{device\_map="auto"}.

Also, the amount of memory from the GPUs has an impact.
For example, \hfinference{} achieves to store all weights from CodeLlama-70b in the eight A100, each with 40Gb, however,  it cannot do that on the eight V100 with 32GB, requiring to store other parameters in the CPU. This has an impact on the \throughput{} (1.79 vs 0.21), beyond the technilogical improvements introduced by the A100.


\subsection{Correlation between \throughput{}, HumanEval Score, and parameters}

Table \ref{tab:minMaxMetricAutoHFVLLMOnlineInferece} shows that, for both \hfinference{} and \vLLM{}, those that maximize the \throughput are the models with smaller number of params, such as Bloom-1b7, Gemma-2, and Starcoder2-3b.
%Having fewer parameters involves to execute less floating point operation and thus to return faster the results.
%We compute the correlation between parameters and \throughput (columns HF Best, vLLM Same and vLL Best).
The Pearson correlation between parameters and   \throughput (columns HF Best, vLLM Same and vLL Best) returns coefficients are between -0.623 and -0.67, suggesting noticeable inverse relationship between throughput and the number of parameters (p-values between 0.001 and 0.003). 
%This means that as the number of parameters increases, the throughput tends to decrease, and this relationship is relatively strong but not perfect.
%At the significant level $\alpha=0.05$,  the correlation is significant, in all the cases ).

We also analyze the trade-off between model size and \throughput{}.
Largest models generaly achieves the highest performance scores such as pass@1 in HumanEval, as shown in \autoref{tab:model_data}.
The correlation coefficient between HumanEval  and parameters is 0.527 (p-value 0.017), indicating a moderate positive relationship. This suggests that models with more parameters tend to have higher HumanEval scores. 
%A hypothesis test was conducted to assess the significance of this correlation. Since we rejected the null hypothesis, we conclude that there is a statistically significant correlation between HumanEval scores and the number of parameters
We also compare the correlation between \throughput{} and HumanEval.
For \hfinference{} the coefficient is $-0.58$ (p-value 0.0072). As throughput  increases, HumanEval tends to decrease.
%Since the p-value is less than the  significance level $\alpha=0.05$, this correlation is  statistically significant.
For \vLLM{}, considering the `best' \throughput{} (\autoref{tab:minMaxMetricAutoHFVLLMOnlineInferece})  the coefficient is -0.35 (p-value 0.122): As throughput increases, HumanEval tends to decrease slightly. At the significant level $\alpha=0.05$, the correlation is not significant.
These results suggest that \vLLM{} achieves a more favorable trade-off between performance and throughput compared to \hfinference.



\subsection{Threats to Validity}

HumanEval not be representative for code completion task.

Inference with other engines.

other parameters that affects \throughput{} that we do not focus.
We focus on two


\section{Related work}
\label{sec:relatedwork}


%\subsection{Inference engines}

%\cite{kwon2023vllmBlog} comparison HF and vLLM.
%\cite{yu2023characterizing} 
%\subsection{HP0}

Wang et al. \cite{wang23HOPLLM} presented EcoOptiGen, a  hyperparameter optimization for LLM inference.
Their and our work have suntantial differences.
They hyperoptimize the inference of closed-LLM from OpenAI, accesible through an API with the goal at optimizing accuracy.
On the contrary, our work focus on performance (througput) by exploring parameters such as number of GPUs, batch sizes, which are not accessible via the OpenAI API, and we focus on optimizing open LLMs. 

Our work focus optimize hyperparameter in order to avoid issues such as out of memory during inference. 
Previous work have study inference issues.
For example,   Gao et al. \cite{Gao2024GPUlowIcse}  studied low GPU utilization issues from jobs submitted to Platform-X, Microsoft’s internal deep learning platform.
They classified 706 issues discovered across 400 deep learning jobs, and found that the 25.64\% of the issues were related to ``Improper Batch Size'' and 
the 3.12\% are related to ``Insufficient GPU Memory".  
Zhang et al. \cite{Zhang2020FailuresJobs} conducted a similar study another deep learning platform in Microsoft (Philly) and found that 8.8\% of the issues were related to GPU out of memory.
These results shows that \approachhpo{} (after changing the fitness function as we discuss in Future work Section \ref{sec:fw}) could be potentially useful to avoid these type of issues.
Motivated by the out of memory failures, tools such as DNNMem~\cite{Gao2020EstimatingGPUconsumption} and DNNPerf~\cite{Gao2023RuntimePerformancePrediction}  were proposed for predicting  GPU memory consumption and performance of deep learning models. 
Similarly, Cao et al. \cite{cao2022understanding} studied performance problems of TensorFLow and Keras frameworks from 210 StackOverflow posts.
They found 12 performance problem related to ``Improper Hyper Parameter''.  
In future work, \approachhpo{}  could be adapted to try to fix them.
%Note that none of these worked focused on large language models.

Previous work have also focused on studying training and/or inference configuration via hyperparameters.
McCandlish et al. \cite{mccandlish2018empirical} predicted the largest useful batch size for neural network training, addressing the trade-off between training speed and computational efficiency. In our paper, we focus on inference.
Gao et al.~\cite{gao2021resource} proposed DnnSAT, a resource-guided AutoML approach for deep learning models to help existing AutoML tools ~\cite{hutter2019automated} (such as Hyperparameter Optimization)  efficiently reduce the configuration space.
%They  evaluate the reduction effectiveness of DnnSAT on two models (not LLMs)  achieving of a reduction of the configuration space up to 53.4\% and 24.1\% respectively.  
DnnSAT could eventually be integrated into our tool \approachhpo{} to reduce the number of configurations.
%Islam et al.~\cite{islam2019comprehensive}  study of bugs in the usage of deep learning libraries inclucuding TensorFlow and Torch by analyzing StackOverflow post and commits. They found that Incorrect Model Parameter is one of the most of the bugs happen in the Data Preparation stage of the deep learning pipeline.
%These kind of problems can be solved by some automated model and parameter recommendation tools.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Previous work have conducted related empirical works  on LLM inferences as our, but with different goals.
For example, Samsi et al. \cite{Samsi2023BenchmarkingInferenceLlama} bechmarked the energy consumed by Meta Llama models: 7B, 13B and 65B.
%As we do, they executed the experiments in \nvidia{} A100 and V100 and varied the batch size.
Beyond the research goals, there are some differences with our work, notatly the model evaluated (3 vs 20) and the inference libraries (Llama scripts~\cite{llamaScripts}, based on Pytorch and  FairScale \cite{FairScale2021}, vs \hfinference{} and \vLLM{})
Argerich et al. \cite{Argerich2024Inference} presented a EnergyMeter, a software based tool easuring the energy consumption of different hardware
components. For evaluate it,  they considered LLMs with at most 7b parametrs (we consider models up to 70b) and used HuggingFace Transformers for inference.
%
Coignion et al.~\cite{coignion:hal-04525620} evaluated the code generated by 18 LLMs on Leetcode benchmark. 
The main difference with our work, beyond the goal, are the model evaluated (they consider smaller LLMs, up to 15b parameters) and the inference engine used (DeepSpeed vs \hfinference and \vLLM{).
Yarally et al. \cite{Yarally2023BatchingGreenAI}  studied how batch inference affect the energy consumption of computer vision tasks using Pytorch.
Alizadeh et al \cite{alizadeh2024green} evaluated the  energy consumption of deep learning  runtime infrastructures such as ONNX,  PyTorch and TensorFlow. They also considered two batch sizes (1 and 64). 
Beyond the differences on the research  goals, these two works do not focus on LLMs.




%\subsection{Hyperparameter optimizations}




%\cite{juravsky2024hydragen} inference
%https://github.com/ScalingIntelligence/hydragen

%\cite{wang2024q}


%%% https://lmsys.org/blog/2024-07-01-routellm/ 
%\cite{ong2024routellmlearningroutellms} 
%\cite{chiang2024chatbot}


% https://vast.ai/pricing

%\redtext{\cite{bavarian2022efficient}????}


% LLMCarbon: Modeling the End-to-End Carbon Footprint of Large Language Models

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%The paper Language Models for Code Completion: A Practical Evaluation, not already put in arxiv may e interesting.
%https://conf.researchr.org/details/icse-2024/icse-2024-research-track/138/Language-Models-for-Code-Completion-A-Practical-Evaluation



%\cite{sukthanker2024hw} hardware aware energy

%out of scope
%\cite{vartziotis2024learn}Learn to Code Sustainably: An Empirical Study on LLM-based Green Code Generation
%\cite{yuan2023rethinking} LLM for mobile, with energy consumption.
%%%\cite{espejel2024low} out of cope
%\cite{Luccioni2023EnergyBloom} energy of training and inference with real calls.
% ML models has focused on estimating the CO2 emissions produced by generating the electricity necessary for powering model training – this is typically referred to as dynamic consumption.
%broader infrastructure that maintains and connects this hardware also requires large amounts of energy to power it – this is referred to as idle consumption.

 %% I like the difference of energy: Iddle, Dynamic, as we have done in GreenRepair with Net Gross.

%  The model received an average of 558 requests per hour, which were handled in real time (i.e. without any batching), for 230,768 requests in total.

%https://github.com/bigscience-workshop/carbon-footprint/



%%LLMCARBON: MODELING THE END-TO-END CARBON FOOTPRINT OF LARGE LANGUAGE MODELS
%https://github.com/sotarokaneda/mlcarbon

%\cite{yang2024robustness} Survey: Robustness, security, privacy, explainability, efficiency, and usability of large language models for code



%% Sharding
% https://engineering.fb.com/2021/07/15/open-source/fsdp/
%oos
%\cite{Everman2023CarbonImpactLLM} very related work. Use 10 prompts on GTPs-families.
%% out of scope
%\cite{zheng2024correctnessbenchmarkingmultidimensionalcode} Beyond Correctness: Benchmarking Multi-dimensional Code Generation for Large Language Models

%%they compute energy and througput, but we can ignore it
%%\cite{mortier2024hybrid,wilkins2024hybrid} very related, eva inference of LLama and Mistral.
%% interesting but out of scope
%\cite{luccioni2023power} very related. 
%Also focus on different tasks including text generation.
%oos
%\cite{izadi2024language} Language Models for Code Completion: A Practical Evaluation

%\cite{Konishi2024EfficientLlama2}

%\cite{yu2024opencarboneval} Important: carbon estimation of LLM.

%oos
%\cite{huang2024soap} very related work

%oos
%%%\cite{Babakol2024TensorEnergy} important
%oos
%%\cite{cunningham2024efficient}
%%oos
%\cite{qiu2024efficient}



%\cite{ahmed2024studyingClosedOpen} Closed open


%\cite{ma2024era} 1bit energy


%oos
%\cite{Li2023CloverInverenceService} 
%ood
%\cite{Hort2023EnergLLMySLR} energy of LLM 

%\cite{Henderson2020SystematicEnergyML}

%\cite{chen2021evaluating} Humman-Eval.


%%\cite{hidvégi2024cigar} reduction of price per token.
%\cite{patel2023polca} power of cloud


%\cite{berthelot2024ImpactGenAI}
%quite related: focus on g5k 

%\subsection{Optimizations}

%\cite{zhang2023ecoassistant}


%%% David low
%\cite{Shi2023greening}


%%% CAIN Paper:

%%GROC

%\cite{wu2024benchmarking} benchamring interaction code gen
%\cite{deng2024r2c2benchmarkCodeGen} benchmarking code gen

%\cite{jiang2024effectiveness}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Conclusions and Future work}
\label{sec:conclusion}
\label{sec:fw}

In this paper, we conduct a large-scale evaluation of the \throughput{} of 20 LLMs using two inference engines.
We inspect the \throughput landscape from the hyperparameter space and demonstrate that hyperparameter optimization can be applied to improve \throughput{}.

In future work, we plan to:
\begin{inparaenum}[\it 1) ]
\item Evaluate the performance of other inference engines such as those listed in the surveys~\cite{miao2023towards,zhou2024survey}.
\item Analyze the landscapes from other measures such as resource utilization (CPU, GPU)  or latency. 
\item Incorporate these measures into \approachhpo{} to add them to the optimization objective (fitness function).
\item Evaluate other hyperparameter optimization approaches and space reduction techniques such as \cite{cao2022understanding} 
\item Study and optimize others hyperparameters that may affect \throughput{} and the eventual new measures.
\item Incorporate the specification of these hyperparameter spaces into \approachhpo{}.
\item Release a usable version of \approachhpo{} (beyond its current status of research prototype) and present its architecture, design and implementation decisions, and usage in a demo/tool track paper.

\end{inparaenum}






\bibliographystyle{plain}
\bibliography{references.bib}

%\newpage
%\appendix
%\input{appendix}


\end{document}


\begin{comment}
https://conf.researchr.org/track/icse-2025/icse-2025-research-track
    
    i) Novelty: The novelty and innovativeness of contributed solutions, problem formulations, methodologies, theories, and/or evaluations, i.e., the extent to which the paper is sufficiently original with respect to the state-of-the-art.

ii) Rigor: The soundness, clarity, and depth of a technical or theoretical contribution, and the level of thoroughness and completeness of an evaluation.

iii) Relevance: The significance and/or potential impact of the research on the field of software engineering.

iv) Verifiability and Transparency: The extent to which the paper includes sufficient information to understand how an innovation works; to understand how data was obtained, analyzed, and interpreted; and how the paper supports independent verification or replication of the paper’s claimed contributions. Any artifacts attached to or linked from the paper will be checked by one reviewer.
\end{comment}


\section{Introduction}
\todo{cite in the intro \cite{bai2024beyond}\cite{li2024llm}}

%Yarally2023BatchingGreenAI
%The batch size (i.e., the number of input data
%samples that are processed at one time during inference) is
%one of the most important hyperparameters to tune during the
%training phase. It has implications on the model accuracy and
%generalisability [5], training times and parallelisability [13],
%etc.


Xhou et al. \cite{zhou2024survey} survey on efficient inference  for LLMs, which  targets different aspects, from providing primary causes of
the inefficient LLM inference to  defining comprehensive taxonomies of, for instance, inference engines.
In particular, they analyze features from inference engines including the two we consider, \hfinference and \vLLM{}
They also conducted experiments such as the evaluation of the speed-ups achieved
by employing uantization techniques on two models LLaMA-2-7B and 13B using two inference frameworks, TensorRT-LLM\cite{}  and LMDeploy\cite{}. 
Recent advances on inference are also discussed in \cite{li2024llm}
%They used a single single NVIDIA A100 GPU and 
\cite{miao2023towards} survey

\cite{shi2024efficient} to cite, importan vision paper.

\cite{white2023navigating} 
`` The directions highlighted in this section are just examples of the opportunities afforded by the emergence of generative AI and copilots in search settings. There are other areas for search providers to
consider too, such as multilingual copilot experiences (i.e., foundation models are powerful and could help with language translation
[33, 74]), copilot efficiency (i.e., large model inference is expensive and not sustainable at massive scale, so creative solutions are
needed [72]), the carbon impact from running foundation models
at scale to serve billions of answers for copilots [18], making copilots private by design [70],``


\todo{\cite{yang2024robustness} no mention any hpo work on LLM}


\todo{\cite{miao2023towards} survey inference, different to the other}

%\todo{check survey LLM for codegen\cite{jiang2024survey}}


%We are living a era where  artificial intelligence is changing many professions, including software engineering.
%The maner of developers build, test, deploy and maintant has also radicaly change since the apareance of these large language models.

%We are living a era where  artificial intelligence allows developers to do tasks quite 
\todo{High throughput serving of large language models (LLMs)
requires batching sufficiently many requests at a time (vllm paper)}

\todo{\cite{ghadesi2024causes} hyperparameter in SO including HF post.}

Large language models (LLM) have revolutionized the manner in which developers build \emph{intelligent} software solutions, impacting several areas, including most of the software engineering (\cite{}).
One of the main actors from this revolution are the \emph{open-source} LLMs. 
which has publicly accessible architecture, code, checkpoint (model weights) and, eventually, training data.
Open-source LLMs enables developers to create AI-based solutions while maintaining control over aspects such as privacy and compliance, and, at the same type, providing governance and ownership of the model deployment process.
%
The current success of open-source in AI, including open-LLM, could be attributed to platforms such as \hf{} (\hfsig), which offers more than 700.000 models available for download, including state-of-the-art models such as CodeLlama~\cite{roziere2023codellama}.
%

Inference engines (or frameworks) are software components that make LLMs operable.
They have as main responsibility to load the model's weighs into the available devices (GPU and/or CPU), and to make the \emph{inference} i.e., to generate a prediction, output, response based on input data.
\hf{}, for instance, provides inference mechanisms into its \texttt{Transformer} library~\cite{wolf-etal-2020-transformers}, for example \texttt{pipelines}, which are objects that abstract complex code used for inference (wraps other libraries such as Pytorch) and offer a simple API dedicated to several tasks, including text generation.

%The appearance of open-source \llm{} encourages this latter strategy, as a developer can download a model, modify it (e.g. applying fine-tuning, pruning, quantization, or other techniques) and then deploy it in a desired infrastructure as those mentioned.
%For example, \hf{} (\hfsig), the platform that drives open-source initiatives on AI,  has more than 700.000 models available for download.
%To applying this strategy, the developers need an inference engine, which is a piece of software that has as main responsibility to load the model into the available devices (GPU and/or CPU), and then to query it (i.e., to perform the inferences).
%Among all the functionalities and features provided by \hf, there are two that simplify the integration of \llm{} into apps, available on library \texttt{Transformer}~\cite{wolf-etal-2020-transformers}.
%The first one, \texttt{AutoModel.from\_pretrained(<model\_id>)}, downloads and loads a model on the available devices.
%Then, \hf{} provides different methods for performing inference on that loaded model, such as \texttt{pipelines}, which offer a simple API dedicated to several tasks, including text generation.
%For instance, \hf{} provides \texttt{pipelines}, which are objects that abstract complex code used for inference (which wraps other libraries such as PyTorch) and offer a simple API dedicated to several tasks, including Text-Generation.
%\hf{} pipelines simplifies the manner to integrate and use \llm{} within software application.  

A key factor for the success of an inference engine is \emph{performance}, because it directly impacts the user experience of AI-powered systems.
%Inference engines are critical components in the deployment of \llm{} into real-world applications. 
%Their performance directly impacts the user experience of AI-powered systems.
A measure of LLM performance is \emph{\throughput{}}, expressed in tokens generated by \llm{} per unit of time.
%Measurement of the performance of an inference engine involves evaluating various metrics such as \emph{\throughput{}}, expressed in tokens generated by an \llm{} per unit of time.
%This metric represents the number of inferences that the inference engine can process per unit of time or, in the case of text generation tasks, the amount of text (expressed as the number of tokens) per unit of time that \llm{} can generate.
%High throughput indicates the engine can handle a large volume of requests efficiently or can generate t.
With the goal of improving the performance of the inference process, inference engines have recently emerged~\cite{miao2023towards,zhou2024survey}, for example, \vLLM{}~\cite{kwon2023efficient}, a memory-efficient inference engine for \llm{}, launched in June 2023.
Inference engines such as vLLM or HuggingFace can be integrated into applications with a few lines of code, as \autoref{lsthf1} shows.
However, the inference engine has hyperparameters that developers need to set by the developers.
Listing \ref{lsthf1} shows a real utilization of \hf{} pipelines\footnote{\url{https://github.com/adit-copilot/EnchantedQuest/blob/48d6256c482abc40a8c916c6c8d1a7c5edb2c6fa/retrival/qa_pipeline.py\#L46}}, which first loads the model (it has one hyperparameter \texttt{device\_map}) and then creates a pipeline with the model as a parameter. % together with other hyperparameters (e.g,  \texttt{max\_new\_tokens}). 
Listing~\ref{lstvll1} shows  real code (but simplified)  that uses \vLLM{}\footnote{\url{https://github.com/tencent-ailab/persona-hub/blob/5e9b7d0a29eff2e2eaf01cc8c74d4abb731fb4a0/code/vllm\_synthesize.py\#L37}}. 
The first line loads the model (with hyperparameter \texttt{tensor\_parallel\_size}), the second performs inferences from a list of prompts (receives two hyperparameter \texttt{temperature} and  \texttt{top\_p}).


\begin{lstlisting}[language=Python, caption=\mbox{\hf{}},
 basicstyle=\tiny, %or \small or \footnotesize etc.
label=lsthf1
]
    model = AutoModelForCausalLM.from_pretrained(model_name, device_map='auto',[...])
    return pipeline("text-generation", 
        model=model, 
        max_new_tokens=100,
        model_kwargs={"torch_dtype": torch.bfloat16} [...]
    )
\end{lstlisting}





\begin{lstlisting}[language=Python, caption=\mbox{\vLLM{}},
 basicstyle= \tiny, %or \small or \footnotesize etc.
label=lstvll1
]
    llm = LLM(model=model_path, tensor_parallel_size=4)
    #tensor_parallel_size based on the GPUs you are using
    outputs = llm.generate(prompts, SamplingParams(temperature=0.6, top_p=0.95, [...]))
\end{lstlisting}


%From the listings we observe that both libraries have \emph{hypermarameters}.
%Listing \ref{lstvll1} shows three, one used on model load  (\texttt{tensor\_parallel\_size=4}) and other two are used during inference (\texttt{temperature=0.6} and  \texttt{top\_p=0.95}).


There are hyperparameters that have a direct incidence in \throughput{} while others do not (for example, \texttt{temperature} affects the output of an \llm{}).
%
{{In this paper, we study the impact of hyperparameters on \throughput{}.}}

Before continuing, let us briefly describe some of these hyperparameters.
\texttt{tensor\_parallel\_size} from \vLLM{} is the number of GPUs to use for distributed execution with tensor parallelism.\footnote{\url{https://github.com/vllm-project/vllm/blob/main/vllm/entrypoints/llm.py\#L44C9-L44C29}}
The \texttt{tensor\_parallel\_size} value needs to be set by the developer according to the resources available in the deployment infrastructure.
In \autoref{lstvll1}, \texttt{tensor\_parallel\_size} is hard-coded to 4. In fact, the initialization of the inference engine \vLLM{} is followed by the following comment:
\emph{\#tensor\_parallel\_size based on the GPUs you are using}.
Both \texttt{from\_pretrained} and \texttt{pipeline} form \hf{} have a similar hyperparameter, named \texttt{device\_map},  which indicates the devices (GPU, CPU) to use.
In Listing\ref{lsthf1}, \texttt{device\_map} receives the value \texttt{auto}, which means that \hf{}  automatically determines the deployment of the model depending on the available resources. %CUDA_VISIBLE_DEVICES


Another of these hyperparameters that affect \throughput{} is \emph{batch size}, which refers to the number of input instances processed simultaneously by the model in a single inference call. 
Increasing the batch size typically increases throughput.
However, this is subject to the limitations of the memory capacity of the hardware (e.g., GPU is not able to allocate the memory of numerous inputs).
On the other hand, a low value may lead to hardware being underutilized.
For example, \autoref{lsthf2batch} shows a snippet from a real app\footnote{\url{https://github.com/mlcommons/inference/blob/c3c68ee61896e1e4d74b096565b627e14422337d/language/mixtral-8x7b/SUT.py\#L130}}
 that sets the \texttt{batch\_size} with the value given by the user, but if it is not provided, the default value $32$ is set. 

\begin{lstlisting}[language=Python, caption=\mbox{},
 basicstyle=\tiny, %or \small or \footnotesize etc.
label=lsthf2batch
]
     if not batch_size:
            if device == "cpu":
                batch_size = 1
            else:
                batch_size = 32  # Reduce to 8 if using 4 GPUs, 16 for 8.
        self.batch_size = batch_size
\end{lstlisting}

%\todo{Choosing an appropriate batch size $n$ is challenging.
%On the one hand, a high value of batch size would lead optimize the resource (GPU) utilization and, consequently, increase the throughput, expressed in tokens per second.
%However, at the same time, a high batch size may lead to an out-of-memory exception: for example, the GPU is not able to allocate the memory of numerous inputs.
%On the other hand, a low value may lead to resources (e.g., GPUs) being underutilized.}


The problem is that \llm{} have different hardware (GPUs) and memory requirements (e.g., VRAM memory). For instance, some LLMs need to be distributed across multiple GPUs to manage their size and the computational load.
Consequently, letting developers choose and set hyperparameter values, especially the number of GPUs and batch size, may have negative effects on the inference performance. 


The final goal of our research is to equip developers with approaches and tools for hyperparameter optimization to achieve high-performance inference.

In this paper, we first study how hyperparameters of inference engines affect  the \throughput{}of \llm{}.
In particular, we examine the throughput landscape defined by the spaces of two hyperparameters, the number of GPUs and batch size.
We study it in the context of code generation: we exercise \llm{} with the code completion task, where each inference consists of completing the code given as input. 

In our experiment, we consider 20 open-source \llm{}, all from key players in the AI industry such as Meta, Google, Microsoft, Mistral and HuggingFace, 
and we use \hfinference{} and \vLLM{} as inference engines.
The experimental infrastructure used is equipped with 8 GPUs \nvidia{} A100 and 8 \nvidia{} V100, which are devices used to train and evaluate most of the \llm{} under consideration.


The results shows 

\todo{}



We also present an approach for hyperparameters optimization.


The paper continues as follows.
Section \ref{}.
Section \ref{}.
Section \ref{}.
Section \ref{}.
Section \ref{}.
Section \ref{}.


==> old/figBatchSizeAll.tex <==
\begin{figure*}
\centering

                    \begin{subfigure}{0.45\textwidth}
                        \centering
                        \includegraphics[width=0.9\textwidth]{plots/plot_RQ3_bs_totalEnergyJ_tesla_vLLM.pdf}
                        \caption{totalEnergyJ tesla vLLM}
                        \label{fig:RQ3_bs_totalEnergyJ_tesla_vLLM}
                    \end{subfigure}
                     \begin{subfigure}{0.45\textwidth}
                        \centering
                        \includegraphics[width=0.9\textwidth]{plots/plot_RQ3_bs_totalEnergyJ_a100_vLLM.pdf}
                        \caption{totalEnergyJ a100 vLLM}
                        \label{fig:RQ3_bs_totalEnergyJ_a100_vLLM}
                    \end{subfigure}
                    

                    \begin{subfigure}{0.45\textwidth}
                       \centering
                        \includegraphics[width=0.9\textwidth]{plots/plot_RQ3_bs_totalEnergyJ_tesla_autohf.pdf}
                        \caption{totalEnergyJ tesla autohf}
                        \label{fig:RQ3_bs_totalEnergyJ_tesla_autohf}
                    \end{subfigure}
                     \begin{subfigure}{0.45\textwidth}
                        \centering
                        \includegraphics[width=0.9\textwidth]{plots/plot_RQ3_bs_totalEnergyJ_a100_autohf.pdf}
                        \caption{totalEnergyJ a100 autohf}
                        \label{fig:RQ3_bs_totalEnergyJ_a100_autohf}
                    \end{subfigure}
                    

                    \begin{subfigure}{0.45\textwidth}
                        \centering
                        \includegraphics[width=0.9\textwidth]{plots/plot_RQ3_bs_throughput_tesla_vLLM.pdf}
                        \caption{throughput tesla vLLM}
                        \label{fig:RQ3_bs_throughput_tesla_vLLM}
                    \end{subfigure}
                      \begin{subfigure}{0.45\textwidth}
                        \centering
                        \includegraphics[width=0.9\textwidth]{plots/plot_RQ3_bs_throughput_a100_vLLM.pdf}
                        \caption{throughput a100 vLLM}
                        \label{fig:RQ3_bs_throughput_a100_vLLM}
                    \end{subfigure}
                    

                    \begin{subfigure}{0.45\textwidth}
                        \centering
                        \includegraphics[width=0.9\textwidth]{plots/plot_RQ3_bs_throughput_tesla_autohf.pdf}
                        \caption{throughput tesla autohf}
                        \label{fig:RQ3_bs_throughput_tesla_autohf}
                    \end{subfigure}
                    \begin{subfigure}{0.45\textwidth}
                        \centering
                        \includegraphics[width=0.9\textwidth]{plots/plot_RQ3_bs_throughput_a100_autohf.pdf}
                        \caption{throughput a100 autohf}
                        \label{fig:RQ3_bs_throughput_a100_autohf}
                    \end{subfigure}
                    

                    \begin{subfigure}{0.45\textwidth}
                        \centering
                        \includegraphics[width=0.9\textwidth]{plots/plot_RQ3_bs_energyJPerToken_tesla_vLLM.pdf}
                        \caption{energyJPerToken tesla vLLM}
                        \label{fig:RQ3_bs_energyJPerToken_tesla_vLLM}
                    \end{subfigure}
                      \begin{subfigure}{0.45\textwidth}
                        \centering
                        \includegraphics[width=0.9\textwidth]{plots/plot_RQ3_bs_energyJPerToken_a100_vLLM.pdf}
                        \caption{energyJPerToken a100 vLLM}
                        \label{fig:RQ3_bs_energyJPerToken_a100_vLLM}
                    \end{subfigure}
                    

                    \begin{subfigure}{0.45\textwidth}
                        \centering
                        \includegraphics[width=0.9\textwidth]{plots/plot_RQ3_bs_energyJPerToken_tesla_autohf.pdf}
                        \caption{energyJPerToken tesla autohf}
                        \label{fig:RQ3_bs_energyJPerToken_tesla_autohf}
                    \end{subfigure}
                     \begin{subfigure}{0.45\textwidth}
                        \centering
                        \includegraphics[width=0.9\textwidth]{plots/plot_RQ3_bs_energyJPerToken_a100_autohf.pdf}
                        \caption{energyJPerToken a100 autohf}
                        \label{fig:RQ3_bs_energyJPerToken_a100_autohf}
                    \end{subfigure}
                    
\caption{}
\label{fig}
\end{figure*}

==> old/tabRq1BothEngine.tex <==
\begin{table*}[t]
    \centering

    \caption{Caption}
    \label{tab:rq1}

\begin{tabular}{l|rrrr|rrrr|rrrr}
\toprule
 & \multicolumn{4}{r}{energyJPerToken} & \multicolumn{4}{r}{throughput} & \multicolumn{4}{r}{totalEnergyJ} \\
engine & \multicolumn{2}{r}{autohf} & \multicolumn{2}{r}{vLLM} & \multicolumn{2}{r}{autohf} & \multicolumn{2}{r}{vLLM} & \multicolumn{2}{r}{autohf} & \multicolumn{2}{r}{vLLM} \\
hardware & a100 & tesla & a100 & tesla & a100 & tesla & a100 & tesla & a100 & tesla & a100 & tesla \\
model &  &  &  &  &  &  &  &  &  &  &  &  \\
\midrule
starcoder & 450.2 & 1034.4 & 9.4 & 23.8 & 0.3 & 0.2 & 32.5 & 22.3 & 1705142 & 4579650 & 48459 & 123075 \\
starcoder2-3b & 10.8 & 14 & 3.1 & 5.6 & 26.6 & 21.8 & 104.1 & 57.1 & 55607 & 72241 & 16118 & 29125 \\
starcoder2-7b & 19.1 & 26 & 5.3 & 10.6 & 15.7 & 12.4 & 61.1 & 31.4 & 97617 & 132285 & 27499 & 54922 \\
CodeLlama-13b-hf & 205.7 & 502.2 & 8.5 & 19.6 & 0.7 & 0.3 & 35.4 & 16.1 & 1062532 & 2593770 & 43737 & 101420 \\
CodeLlama-34b-hf & 1531.6 & 2491 & 33.5 & 51.4 & 0.1 & 0.1 & 32.4 & 17.5 & 7910871 & 12866023 & 172899 & 265252 \\
CodeLlama-7b-hf & 18.8 & 25.2 & 5 & 10.3 & 15.7 & 12.3 & 63 & 31.2 & 97611 & 130318 & 26040 & 53401 \\
gemma-2b & 9.3 & 12.9 & 2.5 & TO & 28.8 & 22 & 132.3 & TO & 47623 & 66024 & 13028 & TO \\
gemma-7b & 75.3 & TO & 14.3 & TO & 2.1 & TO & 70.8 & TO & 372834 & TO & 74043 & TO \\
microsoft\_phi-1\_5 & 6.7 & 9.1 & 1.9 & 3 & 37 & 28.6 & 171.5 & 110.9 & 34317 & 46490 & 9974 & 15473 \\
Mistral-7B-v0.1 & 20.5 & 26.8 & 5.1 & 10.9 & 14.3 & 11.5 & 62.3 & 30 & 105672 & 137500 & 26229 & 56369 \\
Mixtral-8x7B-v0.1 & 518.6 & TO & TO & TO & 0.7 & TO & TO & TO & 2598995 & TO & TO & TO \\
\bottomrule
\end{tabular}

\end{table*}

==> tables/olds/tabInferenceHF.tex <==
\begin{table*}[t]
    \centering

    \caption{RQ1: Online inference (Batch size = 1)}
    \label{tab:rqinferenceHF}

\begin{tabular}{l|rr|rr|rr}
\toprule
 & \multicolumn{2}{r}{e/t} & \multicolumn{2}{r}{throughput} & \multicolumn{2}{r}{totalEnergyJ} \\
engine & \multicolumn{2}{r}{autohf} & \multicolumn{2}{r}{autohf} & \multicolumn{2}{r}{autohf} \\
hardware & a100 & tesla & a100 & tesla & a100 & tesla \\
model &  &  &  &  &  &  \\
\midrule
CodeLlama-13b & 171.5 & 502.2 & 0.7 & 0.3 & 886,002 & 2,593,770 \\
CodeLlama-34b & 1,204 & 2,491 & 0.1 & 0.1 & 6,218,862 & 12,866,023 \\
CodeLlama-7b & 16.9 & 25.2 & 15.7 & 12.3 & 87,302 & 130,318 \\
Mistral-7B-v0.1 & 18.4 & 26.8 & 14.3 & 11.5 & 94,502 & 137,500 \\
Mixtral-8x7B-v0.1 & 1,315.6 & 1,666.7 & 0 & 0.1 & 6,794,859 & 8,178,238 \\
gemma-2b & 8.2 & 12.9 & 28.8 & 22 & 41,661 & 66,024 \\
gemma-7b & 75.3 & 151.3 & 2.1 & 1.2 & 372,834 & 774,527 \\
phi-1 & 5.8 & 9.1 & 37 & 28.6 & 29,531 & 46,490 \\
starcoder & 333.8 & 1,034.4 & 0.3 & 0.2 & 1,264,198 & 4,579,650 \\
starcoder2-3b & 9.7 & 14 & 26.6 & 21.8 & 49,633 & 72,241 \\
starcoder2-7b & 17.3 & 26 & 15.7 & 12.4 & 88,246 & 132,285 \\
\bottomrule
\end{tabular}

\end{table*}



==> tables/olds/tabInferencevLLMComparisonHF.tex <==
\begin{table*}[t]
    \centering

    \caption{Comparison Performance AutoHF vs vLLM. Batch size = 1, Token Generation = 5.}
    \label{tab:inferencevLLMComparisonHF}

\begin{tabular}{l|rl|rl|rl|rl|rl|rl}
\toprule
 & \multicolumn{4}{r}{energyJPerToken} & \multicolumn{4}{r}{throughput} & \multicolumn{4}{r}{totalEnergyJ} \\
hardware & \multicolumn{2}{r}{a100} & \multicolumn{2}{r}{tesla} & \multicolumn{2}{r}{a100} & \multicolumn{2}{r}{tesla} & \multicolumn{2}{r}{a100} & \multicolumn{2}{r}{tesla} \\
engine & vLLM & zDiff & vLLM & zDiff & vLLM & zDiff & vLLM & zDiff & vLLM & zDiff & vLLM & zDiff \\
model &  &  &  &  &  &  &  &  &  &  &  &  \\
\midrule
CodeLlama-13b & 7.6 & -95.6\% & 19.6 & -96.1\% & 35.4 & 49.6X & 16.1 & 52.7X & 39,108 & -95.6\% & 101,420 & -96.1\% \\
CodeLlama-34b & 32.3 & -97.3\% & 51.4 & -97.9\% & 32.4 & 323.0X & 17.5 & 174.0X & 166,825 & -97.3\% & 265,252 & -97.9\% \\
CodeLlama-7b & 4.4 & -74.0\% & 10.3 & -59.1\% & 63 & 3.0X & 31.2 & 1.5X & 22,926 & -73.7\% & 53,401 & -59.0\% \\
Mistral-7B-v0.1 & 4.5 & -75.5\% & 10.9 & -59.3\% & 62.3 & 3.4X & 30 & 1.6X & 23,018 & -75.6\% & 56,369 & -59.0\% \\
Mixtral-8x7B-v0.1 & 19.6 & -98.5\% & 38.5 & -97.7\% & 59.2 & infX & 37 & 369.0X & 101,283 & -98.5\% & 198,839 & -97.6\% \\
gemma-2b & 2.1 & -74.4\% & 4.2 & -67.4\% & 132.3 & 3.6X & 82.3 & 2.7X & 11,074 & -73.4\% & 21,495 & -67.4\% \\
gemma-7b & 6.5 & -91.4\% & 12.8 & -91.5\% & 50.9 & 23.2X & 25 & 19.8X & 33,632 & -91.0\% & 65,991 & -91.5\% \\
phi-1 & 1.6 & -72.4\% & 3 & -67.0\% & 171.5 & 3.6X & 110.9 & 2.9X & 8,241 & -72.1\% & 15,473 & -66.7\% \\
starcoder & 8.4 & -97.5\% & 23.8 & -97.7\% & 32.5 & 107.3X & 22.3 & 110.5X & 43,585 & -96.6\% & 123,075 & -97.3\% \\
starcoder2-3b & 2.7 & -72.2\% & 5.6 & -60.0\% & 104.1 & 2.9X & 57.1 & 1.6X & 13,905 & -72.0\% & 29,125 & -59.7\% \\
starcoder2-7b & 4.7 & -72.8\% & 10.6 & -59.2\% & 61.1 & 2.9X & 31.4 & 1.5X & 24,335 & -72.4\% & 54,922 & -58.5\% \\
\bottomrule
\end{tabular}

\end{table*}

==> tables/olds/tabInferencevLLMComparisonHF2.tex <==
\begin{table*}[t]
    \centering

    \caption{Comparison Performance AutoHF vs vLLM. Batch size = 1, Token Generation = 5. \todo{check if we are comparing the same configuration}}
    \label{tab:inferencevLLMComparisonHF}


\begin{tabular}{lllllllllllll}
\toprule
 & \multicolumn{2}{r}{\% CPU} & \multicolumn{2}{r}{\% GPU} & \multicolumn{2}{r}{\% Mem} & \multicolumn{2}{r}{e/t} & \multicolumn{2}{r}{en ef} & \multicolumn{2}{r}{tp} \\
hardware & \multicolumn{2}{r}{a100} & \multicolumn{2}{r}{a100} & \multicolumn{2}{r}{a100} & \multicolumn{2}{r}{a100} & \multicolumn{2}{r}{a100} & \multicolumn{2}{r}{a100} \\
engine & vLLM & zDiff & vLLM & zDiff & vLLM & zDiff & vLLM & zDiff & vLLM & zDiff & vLLM & zDiff \\
model &  &  &  &  &  &  &  &  &  &  &  &  \\
\midrule
CodeLlama-13b & 0.7 & -8.6\% & 81 & 41.3\% & 81.1 & -6.0\% & 7.6 & -95.6\% & 4.7 & 114391.5\% & 35.4 & 49.5X \\
CodeLlama-34b & 1.3 & 71.2\% & 56.3 & 14.1\% & 84.5 & -0.8\% & 32.3 & -97.3\% & 1 & 1380567.4\% & 32.4 & 369.4X \\
CodeLlama-70b & 2.6 & 501.3\% & 61.7 & 237.3\% & 85.4 & -10.2\% & 76.9 & -97.2\% & 0.3 & 766492.9\% & 21.7 & 214.8X \\
CodeLlama-7b & 0.7 & -5.2\% & 70.5 & -21.1\% & 82 & 23.5\% & 4.4 & -73.7\% & 14.2 & 1426.0\% & 63 & 3.0X \\
Codestral-22B-v0.1 & nan & nan\% & nan & nan\% & nan & nan\% & nan & nan\% & nan & nan\% & nan & nanX \\
Mistral-7B-v0.1 & 0.7 & -6.7\% & 71.8 & -18.6\% & 77.3 & 7.9\% & 4.5 & -75.7\% & 14 & 1700.8\% & 62.3 & 3.4X \\
Mixtral-8x7B-v0.1 & 1.1 & 285.9\% & 45.6 & 192.9\% & 82.8 & 13.0\% & 19.6 & -98.5\% & 3 & 9543355.4\% & 59.2 & 1421.5X \\
gemma-2b & 0.6 & -16.3\% & 54.8 & -22.7\% & 81.7 & 207.0\% & 2.1 & -73.7\% & 61.7 & 1646.7\% & 132.3 & 3.6X \\
gemma-7b & 0.3 & -85.4\% & 57.3 & -10.8\% & 81.7 & -8.9\% & 6.5 & -91.3\% & 7.8 & 28324.3\% & 50.9 & 23.6X \\
phi-1 & 0.5 & -21.4\% & 43.1 & -22.9\% & 85.7 & 472.2\% & 1.6 & -72.3\% & 107.5 & 1571.2\% & 171.5 & 3.6X \\
starcoder & 0.7 & 16.7\% & 82.7 & 66.1\% & 84.7 & 0.8\% & 8.4 & -97.5\% & 3.9 & 428505.4\% & 32.5 & 107.4X \\
starcoder2-3b & 0.6 & -15.1\% & 55.1 & -26.7\% & 84.3 & 169.9\% & 2.7 & -72.2\% & 38.7 & 1305.0\% & 104.1 & 2.9X \\
starcoder2-7b & 0.7 & -9.1\% & 71 & -20.4\% & 82.8 & 17.9\% & 4.7 & -72.8\% & 13 & 1330.9\% & 61.1 & 2.9X \\
\bottomrule
\end{tabular}

\end{table*}

==> tables/tabBatchsizeAuto.tex <==
\begin{table}[t]
\centering

\begin{tabular}{llllllllll}
\toprule
batchSize & 1 & 2 & 4 & 8 & 16 & 32 & 64 & 128 & 256 \\
model &  &  &  &  &  &  &  &  &  \\
\midrule
Bloom-1b7 & 37.6 & 54.8 & 66.3 & 71.5 & 73.6 & 70.9 & 94.3 & - & - \\
Bloom-3b & 27.3 & 36.9 & 43.1 & 44.6 & 45.3 & 50.6 & - & - & - \\
Bloom-7b1 & 16.8 & 20.1 & 21.8 & 21.4 & 28.9 & - & - & - & - \\
Codellama-13b-hf & 0.7 & 1.3 & 2.3 & - & - & - & - & - & - \\
Codellama-34b-hf & 0.1 & 0.2 & 0.3 & 0.6 & 1.1 & - & - & - & - \\
Codellama-7b-hf & 15.7 & 17.5 & 19.1 & 19.2 & 23.5 & - & - & - & - \\
Codestral-22b-v0.1 & 0.2 & 0.4 & 0.7 & 1.3 & 2.2 & - & - & - & - \\
Gemma-2b & 28.8 & 37.4 & 44.1 & 45.8 & 44.5 & 47.3 & - & - & - \\
Gemma-7b & 2.1 & 3.6 & 5.4 & 7.2 & - & - & - & - & - \\
Mistral-7b-v0.1 & 14.3 & 16.3 & 17.9 & 18.2 & 17.9 & 19.1 & - & - & - \\
Mixtral-8x7b-v0.1 & 0 & 0.1 & 0.1 & 0.2 & 0.3 & 0.6 & - & - & - \\
Phi-1 & 26.2 & 6.7 & 12.1 & 19 & 29.8 & 41.6 & 50.7 & - & - \\
Phi-1_5 & 37 & 54.3 & 68.6 & 75.4 & 76.1 & 74.4 & 86 & - & - \\
Phi-2 & 19.5 & 2 & 4 & 6.6 & 11.5 & 16.7 & 25.1 & - & - \\
Starcoder & 30.7 & 38 & 46.5 & 52.7 & 55.1 & 62.4 & - & - & - \\
Starcoder2-3b & 44.8 & 79.7 & 130.1 & 191.5 & 262.8 & 282.4 & 264.4 & 250.6 & 280.3 \\
Starcoder2-7b & 15.7 & 18.2 & 20.2 & 19.8 & 19.5 & 17.9 & 22 & - & - \\
Wizardcoder-15b-v1.0 & 0.3 & 0.5 & 0.9 & 1.5 & 2.6 & - & - & - & - \\
Wizardcoder-33b-v1.1 & 0.1 & - & - & - & - & - & - & - & - \\
\bottomrule
\end{tabular}
\caption{ }
\label{tab:batchsize}
\end{table}

==> tables/tabHFMinMaxGPU.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{l|lr|lr|lr|lr|lr|}
\toprule
model & nrGPUs & tr & nrGPUs-2 & Per-GPU & nrGPUs-3 & Per-Mem & nrGPUs-4 & Per-CPU & nrGPUs-5 & gpu-cpu-ratio \\
\midrule
bloom-1b7 & 1 & 37.6 & 1 & 45.6 & 1 & 18.1 & 1 & 0.3 & 8 & 18.6 \\
bloom-3b & 1 & 27.3 & 1 & 57.6 & 1 & 30.4 & 1 & 0.3 & 8 & 22.1 \\
bloom-7b1 & 1 & 16.8 & 1 & 76.6 & 1 & 68.4 & 1 & 0.4 & 8 & 33.5 \\
CodeLlama-13b-hf & 2 & 9.7 & 1 & 57.3 & 1 & 86.4 & 1 & 0.8 & 8 & 26.1 \\
CodeLlama-34b-hf & 4 & 4.1 & 1 & 49.3 & 1 & 85.2 & 1 & 0.7 & 8 & 28.6 \\
CodeLlama-70b-hf & 8 & 1.8 & 4 & 18.3 & 4 & 95.1 & 4 & 0.4 & 8 & 27.5 \\
CodeLlama-7b-hf & 1 & 15.7 & 1 & 89.3 & 1 & 66.4 & 2 & 0.7 & 8 & 24.8 \\
Codestral-22B-v0.1 & 4 & 5.4 & 1 & 62.9 & 2 & 95.9 & 2 & 0.5 & 8 & 28.6 \\
gemma-2b & 1 & 28.8 & 1 & 70.9 & 1 & 26.6 & 4 & 8 & 4 & 1.7 \\
gemma-7b & 4 & 6.4 & 1 & 64.3 & 1 & 89.7 & 4 & 5.7 & 8 & 1.6 \\
Mistral-7B-v0.1 & 1 & 14.3 & 1 & 88.2 & 1 & 71.6 & 2 & 0.7 & 8 & 27 \\
Mixtral-8x7B-v0.1 & 8 & 4.1 & 1 & 15.6 & 4 & 93.7 & 2 & 0.6 & 8 & 16.8 \\
phi-1 & 2 & 29 & 2 & 23.1 & 2 & 8.2 & 2 & 0.3 & 1 & 5 \\
phi-1\_5 & 1 & 37 & 1 & 55.9 & 1 & 15 & 1 & 0.7 & 8 & 14.7 \\
phi-2 & 2 & 22 & 2 & 28.4 & 2 & 14.8 & 2 & 0.4 & 1 & 15.2 \\
starcoder & 1 & 30.7 & 1 & 65.6 & 1 & 75.1 & 2 & 0.8 & 8 & 9.3 \\
starcoder2-3b & 1 & 44.7 & 1 & 33.2 & 1 & 16.2 & 1 & 0.4 & 8 & 10.2 \\
starcoder2-7b & 1 & 15.7 & 1 & 89.2 & 1 & 70.3 & 1 & 0.8 & 8 & 27.4 \\
WizardCoder-15B-V1 & 2 & 8 & 1 & 65.8 & 1 & 83.9 & 2 & 0.5 & 8 & 19.1 \\
WizardCoder-33B-V1.1 & 4 & 1.6 & 1 & 61.1 & 1 & 89.7 & 4 & 3.1 & 4 & 6.7 \\
\bottomrule
\end{tabular}
\caption{ }
\label{tab:minMaxMetricAutoHFOnlineInferece}
\end{table*}




==> tables/tabHardwareComparison.tex <==
\begin{table}[t]
\centering


\begin{tabular}{lrrrr}
\toprule
model & significant & cliff delta & medianImpr & meanImpr \\
\midrule

\bottomrule
\end{tabular}
\caption{Comparison between \nvidia A100 and V100.}
\label{tab:hardwarecomparison}
\end{table}




==> tables/tabInferenceAutoHF.tex <==
\begin{table*}[t]
\centering


\begin{tabular}{l|rrrr|rrrr|rrrr|}
\toprule

&\multicolumn{4}{c}{Th}  &   \multicolumn{4}{c}{GPU \%} &   \multicolumn{4}{c}{Mem Us \%}\\
%nrGPUs & 1_th & 2_th & 4_th & 8_th & 1_gpu & 2_gpu & 4_gpu & 8_gpu \\
model |  nr GPUs & 1 & 2 & 4 & 8 & 1 & 2 & 4 & 8 & 1 & 2 & 4 & 8\\
% &  &  &  &  &  &  &  &  \\
\midrule
CodeLlama-13b-hf & 0.7 & 9.7 & 9.4 & 8.2 & 57.3 & 46.5 & 21.1 & 10.5 & 86.4 & 63.4 & 32.4 & 16.8 \\
CodeLlama-34b-hf & 0.1 & nan & 4.1 & 3.7 & 49.3 & nan & 21.8 & 10.7 & 85.2 & nan & 80.7 & 41.1 \\
CodeLlama-70b-hf & nan & nan & 0.1 & 1.8 & nan & nan & 18.3 & 11.2 & nan & nan & 95.1 & 82.3 \\
CodeLlama-7b-hf & 15.7 & 14.8 & 13.8 & 13.2 & 89.3 & 42.3 & 19.2 & 9.6 & 66.4 & 33.9 & 17.6 & 9.4 \\
Codestral-22B-v0.1 & 0.2 & 0.8 & 5.4 & 4.5 & 62.9 & 34.3 & 20.5 & 9.6 & 88.7 & 95.9 & 54.4 & 27.9 \\
Mistral-7B-v0.1 & 14.3 & 14 & 11.6 & 10.1 & 88.2 & 42.4 & 17.3 & 7.9 & 71.6 & 36.5 & 18.9 & 10.1 \\
Mixtral-8x7B-v0.1 & 0 & 0.1 & 0.7 & 4.1 & 15.6 & 15.3 & 13.2 & 7.1 & 73.2 & 91.3 & 93.7 & 56 \\
WizardCoder-15B-V1.0 & 0.3 & 8 & 7.6 & 6.2 & 65.8 & 39.3 & 20 & 9.7 & 83.9 & 73.8 & 37.6 & 19.4 \\
WizardCoder-33B-V1.1 & 0.1 & nan & 1.6 & nan & 61.1 & nan & 20.4 & nan & 89.7 & nan & 82.4 & nan \\
bloom-1b7 & 37.6 & 27.7 & 24.4 & 32.8 & 45.6 & 23 & 10.8 & 5.5 & 18.1 & 9.7 & 5.4 & 3.2 \\
bloom-3b & 27.3 & 22.1 & 19.4 & 25.3 & 57.6 & 27.6 & 13.9 & 7.1 & 30.4 & 15.8 & 8.6 & 4.7 \\
bloom-7b1 & 16.8 & 16.2 & 14.2 & 12.6 & 76.6 & 38.7 & 19.6 & 9.3 & 68.4 & 34.9 & 18.1 & 9.6 \\
gemma-2b & 28.8 & 3.9 & 10 & 27.6 & 70.9 & 43.8 & 13.4 & 7.3 & 26.6 & 14.1 & 7.6 & 4.2 \\
gemma-7b & 2.1 & 1.6 & 6.4 & 5.6 & 64.3 & 48.8 & 17.3 & 8.8 & 89.7 & 80.4 & 22 & 11.8 \\
phi-1 & 26.2 & 29 & 25.7 & 17.6 & 1.6 & 23.1 & 10.7 & 4.1 & 2.3 & 8.2 & 4.8 & 3 \\
phi-1\_5 & 37 & 36.2 & 33.5 & 27.7 & 55.9 & 27.3 & 10.2 & 4.5 & 15 & 7.5 & 3.8 & 1.9 \\
phi-2 & 19.5 & 22 & 19.5 & 14.4 & 5.1 & 28.4 & 14.3 & 5.7 & 4.2 & 14.8 & 8.1 & 4.7 \\
starcoder & 30.7 & 21.4 & 19.9 & 16.6 & 65.6 & 28 & 13.6 & 6 & 75.1 & 37.7 & 19.5 & 10.4 \\
starcoder2-3b & 44.8 & 33.4 & 29.1 & 22 & 33.4 & 15.8 & 7.4 & 3 & 16.2 & 8.8 & 5.1 & 3.2 \\
starcoder2-7b & 15.7 & 15.4 & 13.2 & 12 & 89.2 & 43.2 & 18.3 & 8.6 & 70.3 & 35.8 & 18.6 & 9.9 \\
\bottomrule
\end{tabular}

\caption{ }
\label{tab:cAutoHFOnlineInferece}
\end{table*}




==> tables/tabInferenceAutoTesla.tex <==

\begin{table}[t]
\centering


\begin{tabular}{| lllllll| }
\toprule
model & GPUs & tp & GPUs & \%GPU & GPUs & U Mem \\
\midrule
bloom-1b7 & 1 & 30.1 & 1 & 61 & 1 & 22.2 \\
bloom-3b & 1 & 21.7 & 1 & 75.7 & 1 & 37.6 \\
bloom-7b1 & 1 & 13.3 & 1 & 91 & 1 & 85.1 \\
CodeLlama-13b & 4 & 7.1 & 1 & 85.5 & 1 & 88.8 \\
CodeLlama-34b & 8 & 2.9 & 1 & 83 & 4 & 96 \\
CodeLlama-70b & 8 & 0.2 & 4 & 19.4 & 4 & 91.1 \\
CodeLlama-7b & 1 & 12.3 & 1 & 85 & 1 & 82.4 \\
Codestral-22B-v0.1 & 4 & 3.9 & 1 & 85.4 & 2 & 96.7 \\
gemma-2b & 1 & 22 & 1 & 69.3 & 1 & 32.9 \\
gemma-7b & 2 & 3.1 & 1 & 82.6 & 1 & 86.9 \\
Mistral-7B-v0.1 & 1 & 11.5 & 1 & 85 & 1 & 89 \\
Mixtral-8x7B-v0.1 & 8 & 3.6 & 1 & 73.4 & 4 & 82.8 \\
phi-1\_5 & 4 & 29.1 & 1 & 52.7 & 1 & 18.3 \\
phi-2 & 4 & 17.1 & 2 & 28.8 & 2 & 18 \\
starcoder2-7b & 1 & 12.4 & 1 & 90.8 & 1 & 87.4 \\
WizardCoder-15B & 2 & 5.9 & 1 & 86.8 & 2 & 91.9 \\
WizardCoder-33B& 8 & 0.3 & 1 & 80.4 & 1 & 96.6 \\
\bottomrule
\end{tabular}


\caption{Tesla}
\label{tab:TeslaAutoHFOnlineInferece}
\end{table}



==> tables/tabInferenceHF.tex <==


\begin{table*}[t]
    \centering

    \caption{RQ1: Online inference (Batch size = 1)}
    \label{tab:rqinferenceHF}


\begin{tabular}{lllllll}
\toprule
 & e/t & en ef & \% CPU & \% GPU & \% Mem & tp \\

\midrule
CodeLlama-13b & 171.54 & 0.00 & 0.81 & 57.34 & 86.35 & 0.70 \\
CodeLlama-34b & 1,204.04 & 0.00 & 0.74 & 49.31 & 85.21 & 0.09 \\
CodeLlama-70b & 2,733.59 & 0.00 & 0.43 & 18.31 & 95.12 & 0.10 \\
CodeLlama-7b & 16.86 & 0.93 & 0.72 & 89.31 & 66.42 & 15.68 \\
Codestral-22B-v0.1 & 608.86 & 0.00 & 0.77 & 57.24 & 88.65 & 0.18 \\
Mistral-7B-v0.1 & 18.37 & 0.78 & 0.72 & 88.22 & 71.61 & 14.27 \\
Mixtral-8x7B-v0.1 & 1,315.56 & 0.00 & 0.29 & 15.57 & 73.25 & 0.04 \\
gemma-2b & 8.15 & 3.53 & 0.70 & 70.89 & 26.61 & 28.79 \\
gemma-7b & 75.27 & 0.03 & 2.31 & 64.27 & 89.68 & 2.07 \\
phi-1 & 5.76 & 6.43 & 0.70 & 55.91 & 14.98 & 37.02 \\
starcoder & 333.77 & 0.00 & 0.64 & 49.78 & 84.08 & 0.30 \\
starcoder2-3b & 9.68 & 2.75 & 0.74 & 75.14 & 31.23 & 26.63 \\
starcoder2-7b & 17.29 & 0.91 & 0.75 & 89.17 & 70.25 & 15.66 \\
\bottomrule
\end{tabular}

\end{table*}


==> tables/tabInferencevLLMComparisonHF.tex <==
\begin{table*}[t]
    \centering

    \caption{Comparison Performance AutoHF vs vLLM. Online inference (Batch size = 1) 
    }
    \label{tab:inferencevLLMComparisonHF}


\begin{tabular}{|l|lrr|lrr|lrr|lrr|}
\toprule
\%\\%model & nrGPUs & tp &  X & GPUs & Per-GPU & \\% & GPUs & Per-CPU & \\\% & GPUs & gpu-cpu-ratio & \\\% \\
\midrule
Model & nrGPUs & throughput & throughputX & nrGPUs-2 & Per-GPU & Per-GPU\% & nrGPUs & Per-Mem & Per-Mem\% \\
\midrule
bloom-1b7 & 1 & 133.1 & 3.5X & 1 & 27.2 & -40\% & 2 & 82.3 & 355\% \\
bloom-3b & 1 & 98.6 & 3.6X & 1 & 35.1 & -39\% & 4 & 83.1 & 173\% \\
bloom-7b1 & 2 & 67.2 & 4.0X & 1 & 50.7 & -34\% & 2 & 83.2 & 22\% \\
CodeLlama-13b-hf & 4 & 48.2 & 5.0X & 1 & 81 & 41\% & 8 & 87 & 1\% \\
CodeLlama-34b-hf & 8 & 34.7 & 8.5X & 4 & 56.3 & 14\% & 8 & 85.3 & 0\% \\
CodeLlama-70b-hf & 8 & 21.7 & 12.1X & 8 & 61.7 & 237\% & 8 & 85.4 & -10\% \\
CodeLlama-7b-hf & 1 & 63 & 4.0X & 1 & 70.5 & -21\% & 8 & 87.2 & 31\% \\
Codestral-22B-v0.1 & 8 & 64.7 & 12.0X & 2 & 62.1 & -1\% & 8 & 83.2 & -13\% \\
gemma-2b & 1 & 132.3 & 4.6X & 1 & 54.8 & -23\% & 1 & 81.7 & 207\% \\
gemma-7b & 4 & 70.8 & 11.1X & 1 & 57.3 & -11\% & 4 & 82.1 & -8\% \\
Mistral-7B-v0.1 & 4 & 66.5 & 4.7X & 1 & 71.8 & -19\% & 4 & 83.4 & 16\% \\
Mixtral-8x7B-v0.1 & 4 & 59.2 & 14.4X & 4 & 45.6 & 192\% & 4 & 82.8 & -12\% \\
phi-1 & 1 & 158.5 & 5.5X & 1 & 26.4 & 14\% & 2 & 86.5 & 955\% \\
phi-1\_5 & 1 & 171.5 & 4.6X & 1 & 43.1 & -23\% & 4 & 86.5 & 477\% \\
phi-2 & 1 & 110.3 & 5.0X & 1 & 36.2 & 27\% & 2 & 87.5 & 491\% \\
starcoder & 8 & 58.4 & 1.9X & 1 & 82.7 & 26\% & 4 & 86.9 & 16\% \\
starcoder2-3b & 1 & 104.1 & 2.3X & 1 & 55.1 & 66\% & 4 & 86.4 & 433\% \\
starcoder2-7b & 4 & 62.3 & 4.0X & 1 & 71 & -20\% & 4 & 86.3 & 23\% \\
WizardCoder-15B-V1 & 8 & 57.3 & 7.2X & 1 & 66.6 & 1\% & 2 & 86.7 & 3\% \\
WizardCoder-33B-V1.1 & 8 & 43.8 & 27.4X & 4 & 60.1 & -2\% & 8 & 77.4 & -14\% \\

\bottomrule
\end{tabular}


\end{table*}

==> tables/tabVariables.tex <==
\begin{table}[t!]
\centering
\begin{tabular}{|l|l|}
\hline
\textbf{Independent variables} & \textbf{Values} \\
\hline
Model Id        & CodeLlama7B, ... (all values in Table \ref{tab:model_data})\\
Inference framework            & \hfinference{}, \vLLM{}\\
Hardware                       & \nvidia A100-40 GB, \nvidia V100-32GB \\
Number GPUs                    & 1, 2, 4, 8\\
Batch size                     & 1, 2, 4, 8, 16, 32, 64, 128, 256, 1028\\
%Max token generation           & 5, 10, 20 \\

\hline
\end{tabular}
\caption{Independent variables of our experiment. %\todo{we can add a column to say in with RQ we discuss about it}
}
\label{tab:indepVar}
\end{table}


%\begin{table*}[t!]
%\centering
%\begin{tabular}{|l|l|}
%\hline
%\textbf{Type} & \textbf{Variables} \\
%\hline
%Independent variables & Model Id (Name + Param), Inference framework, Hardware, Number %\hline
%Dependent variables   & Total Energy, Energy per token, Total time, Throughput, %Execution time, Errors,  \\
%\hline
%\end{tabular}
%\caption{Independent and Dependent Variables}
%\label{tab:variables}
%\end{table*}

%\paragraph{Independent variables}
%\begin{enumerate}[a)]
%    \item Model Id (Name + Param)
%    %\item parameters
%    \item Inference framework
%    \item Hardware
%    \item Number GPUs
%    \item Batch size
%    \item Max token generation
%\end{enumerate}
%\paragraph{Dependent variables}
%\begin{enumerate}[a)]
%    \item Total Energy
%    \item Energy per token
%    \item Total time
%    \item Throughput
%    \item number of errors
%\end{enumerate}

==> tables/tabWSSummary.tex <==
\begin{table*}[t]
    \centering

    \caption{RQ4}
    \label{tab:hardwareSummary}

\begin{tabular}{|l|ll|rrrrrr|}
\toprule
metric & hardware & engine & total & Increase & Decrease & Incr-Decr & Equal & unclasified \\
\midrule
energyJPerToken & a100 & autohf & 11 & 7 & 1 & 3 & - & - \\
energyJPerToken & a100 & vLLM & 11 & 11 & - & - & - & - \\
energyJPerToken & tesla & autohf & 11 & 6 & 3 & 2 & - & - \\
energyJPerToken & tesla & vLLM & 11 & 8 & 1 & - & 1 & 1 \\
\hline
totalEnergyJ & a100 & autohf & 11 & 7 & 1 & 3 & - & - \\
totalEnergyJ & a100 & vLLM & 11 & 11 & - & - & - & - \\
totalEnergyJ & tesla & autohf & 11 & 6 & 3 & 2 & - & - \\
totalEnergyJ & tesla & vLLM & 11 & 8 & 1 & - & 1 & 1 \\
\hline
throughput & a100 & autohf & 11 & 4 & - & 2 & 5 & - \\
throughput & a100 & vLLM & 11 & 7 & 1 & 3 & - & - \\
throughput & tesla & autohf & 11 & 5 & 1 & 1 & 4 & - \\
throughput & tesla & vLLM & 11 & 10 & - & - & - & 1 \\
\bottomrule
\end{tabular}


\end{table*}

==> tables/tabvLLMMinMaxGPU.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{|l|rr|rr|rr|rr|rr|rr|}
\toprule

model & gpus & tp & gpus & e/t & gpus & en ef & gpus & \% GPU &gpus & \% Mem & gpus & \% CPU \\
\midrule
bloom-1b7 & 1 & 133.1 & 1 & 3.8 & 1 & 35.119 & 1 & 27.2 & 2 & 82.3 & 8 & 3.4 \\
bloom-3b & 1 & 98.6 & 1 & 5 & 1 & 19.566 & 1 & 35.1 & 4 & 83.1 & 8 & 3.9 \\
bloom-7b1 & 2 & 67.2 & 1 & 7.8 & 1 & 8.174 & 1 & 50.7 & 2 & 83.2 & 8 & 4 \\
CodeLlama-13b-hf & 4 & 48.2 & 1 & 7.6 & 1 & 4.679 & 1 & 81 & 8 & 87 & 8 & 2 \\
CodeLlama-34b-hf & 8 & 34.7 & 4 & 32.3 & 4 & 1.002 & 4 & 56.3 & 8 & 85.3 & 8 & 2.3 \\
CodeLlama-70b-hf & 8 & 21.7 & 8 & 76.9 & 8 & 0.282 & 8 & 61.7 & 8 & 85.4 & 8 & 2.6 \\
CodeLlama-7b-hf & 1 & 63 & 1 & 4.4 & 1 & 14.193 & 1 & 70.5 & 8 & 87.2 & 8 & 2 \\
Codestral-22B-v0.1 & 8 & 64.7 & 2 & 17.4 & 4 & 2.469 & 2 & 62.1 & 8 & 83.2 & 8 & 1.9 \\
gemma-2b & 1 & 132.3 & 1 & 2.1 & 1 & 61.701 & 1 & 54.8 & 1 & 81.7 & 8 & 1.8 \\
gemma-7b & 4 & 70.8 & 1 & 6.5 & 1 & 7.811 & 1 & 57.3 & 4 & 82.1 & 8 & 1.9 \\
Mistral-7B-v0.1 & 4 & 66.5 & 1 & 4.5 & 1 & 13.983 & 1 & 71.8 & 4 & 83.4 & 8 & 1.9 \\
Mixtral-8x7B-v0.1 & 4 & 59.2 & 4 & 19.6 & 4 & 3.021 & 4 & 45.6 & 4 & 82.8 & 8 & 2 \\
phi-1 & 1 & 158.5 & 1 & 1.8 & 1 & 89.227 & 1 & 26.4 & 2 & 86.5 & 8 & 1.8 \\
phi-1\_5 & 1 & 171.5 & 1 & 1.6 & 1 & 107.498 & 1 & 43.1 & 4 & 86.5 & 8 & 1.8 \\
phi-2 & 1 & 110.3 & 1 & 2.9 & 1 & 37.483 & 1 & 36.2 & 2 & 87.5 & 8 & 1.9 \\
starcoder & 8 & 58.4 & 1 & 8.4 & 1 & 3.856 & 1 & 82.7 & 4 & 86.9 & 8 & 2.1 \\
starcoder2-3b & 1 & 104.1 & 1 & 2.7 & 1 & 38.672 & 1 & 55.1 & 4 & 86.4 & 8 & 1.9 \\
starcoder2-7b & 4 & 62.3 & 1 & 4.7 & 1 & 12.958 & 1 & 71 & 4 & 86.3 & 2 & 1.5 \\
WizardCoder-15B-V1 & 8 & 57.3 & 1 & 10.5 & 2 & 3.27 & 1 & 66.6 & 2 & 86.7 & 8 & 2 \\
WizardCoder-33B-V1.1 & 8 & 43.8 & 4 & 30.1 & 4 & 1.221 & 4 & 60.1 & 8 & 77.4 & 8 & 2 \\
\bottomrule
\end{tabular}
\caption{ vLLM}
\label{tab:minMaxMetricAutoHFOnlineInferece}
\end{table*}



